Modeling Structure with Undirected Neural Networks

Neural networks are powerful function estimators, leading to their status as a paradigm of choice for modeling structured data. However, unlike other structured representations that emphasize the modularity of the problem -- e.g., factor graphs -- neural networks are usually monolithic mappings from inputs to outputs, with a fixed computation order. This limitation prevents them from capturing different directions of computation and interaction between the modeled variables. In this paper, we combine the representational strengths of factor graphs and of neural networks, proposing undirected neural networks (UNNs): a flexible framework for specifying computations that can be performed in any order. For particular choices, our proposed models subsume and extend many existing architectures: feed-forward, recurrent, self-attention networks, auto-encoders, and networks with implicit layers. We demonstrate the effectiveness of undirected neural architectures, both unstructured and structured, on a range of tasks: tree-constrained dependency parsing, convolutional image classification, and sequence completion with attention. By varying the computation order, we show how a single UNN can be used both as a classifier and a prototype generator, and how it can fill in missing parts of an input sequence, making them a promising field for further research.

==> [ICML 2022] Undirected Neural Networks/_experiments_multitask.tex <==
\section{Multitask Learning}

\andre{I promoted this to section}

\andre{so far the results for this task are not  compelling. consider dropping this.}

We also explore UNN for multiple tasks. Figure \ref{fig:factor_graph_multitask} shows the factor graph for a simple multitask setup. 
 
This graph resembles the directed neural network for multitasking. The difference is that for multiple iterations, UNNs can be more powerful for identifying relations between the multiple task labels. When we have more iteration updates,  

 
\begin{figure*}
    \centering
    \includegraphics[width=12cm]{img/factor_graph_multitask.png}
    \caption{Factor graph for a UNN for multiple tasks.}
    \label{fig:factor_graph_multitask}
\end{figure*}



Here we have the following energies:

\begin{equation}
    E_{X,H}(x,h) = -h^{T}Wx
\end{equation}

\begin{equation}
    E_{H,Y_1}(h,y_1) = -y_1^{T}Vh
\end{equation}

\begin{equation}
    E_{H,Y_2}(h,y_2) = -y_2^{T}Uh
\end{equation}

\begin{equation}
    E_{X}(x) = -a^{T}x + A(x)
\end{equation}

\begin{equation}
    E_{H}(h) = -b^{T}h + B(h)
\end{equation}

\begin{equation}
    E_{Y_1}(y_1) = -c^{T}y_1 + C(y_1)
\end{equation}

\begin{equation}
    E_{Y_2}(y_2) = -d^{T}y_2 + D(y_2)
\end{equation}

We minimize the model with respect to $h$, $y_1$, $y_2$ iteratively. 

\begin{equation}
\begin{split}
    h^\star(x,y) = \\
    \argmin_{h}(E(h) + E(x,h) + E(h,y_1) + E(h,y_2)) \\
    = \argmin_h(-b^{T}h + B(h) \\
    - h^{T}Wx - y_1^{T}Vh - y_2^{T}Uh) \\
    = (\nabla B^{*})(Wx + V^{T}y_1 + U^{T}y_2 + b)
\end{split}
\end{equation}

\begin{equation}
\begin{split}
    y_1^{*}(x,h) = \argmin_{y_1}E(h,y_1) \\
    = (\nabla C^{*})(Vh+b_1)
\end{split}
\end{equation}

\begin{equation}
\begin{split}
    y_2^{*}(x,h) = \argmin_{y_2}E(h,y_2) \\
    = (\nabla D^{*})(Uh+b_2)
\end{split}
\end{equation}




We experiment how the multiple updates of energy optimization can benefit when the model is trained for multiple tasks. For this experiment, we use the architecture described in Section~\ref{section:multitask_unn}. 
We use dataset with movie reviews from IMDB \citep{maas-EtAl:2011:ACL-HLT2011}. On of the tasks is classification of the review sentiment. For the second task, inspired by \citet{zhang2021disentangling}, we add the movie genre as a second related task. Ass described in \citet{zhang2021disentangling}, we use movies with genre Horror and Drama, because as this work shows, the review sentiment is correlated with those two genres. Because the genre is not present in the original dataset, we use the movie genres from the IMDB website. \footnote{https://www.imdb.com/interfaces/, file: \textbf{title.basics.tsv.gz}} The reviews in \citet{maas-EtAl:2011:ACL-HLT2011} contain the movie ID from IMDB and by this ID we match the movie genre. We only use the reviews with genre Drama or Horror (excluding the few cases where both labels are present). The training split from the original dataset is kept, and the test split from the original dataset is split randomly into validation and test set. The number of instances is shown on Table~\ref{table:multitask_data}.

\begin{table}[]
    \centering
    \caption{Number of instances in the training and development split for multitask data on IMDB movie reviews sentiment and genre classification.}
    \begin{tabular}{c|c|c}
        \toprule
         \multicolumn{3}{c}{Train}  \\
         \midrule
         & Drama & Horror \\ 
         \midrule
         Positive & 6111 & 897 \\ 
         Negative & 4412 & 2650 \\
         \midrule
         \multicolumn{3}{c}{Test}  \\
         \midrule
         & Drama & Horror \\ 
         \midrule
         Positive & 6100 & 1055 \\ 
         Negative & 4488 & 2599 \\ 
    \end{tabular}
    \label{table:multitask_data}
\end{table}

The input of the model is the review text and the two tasks we predict are the review sentiment and the genre of the movie this review is written for. 
The movie review is passed through a BERT (we use \emph{BERT-Tiny} \tsvm{cite}) and is used as the input $x$, and the architecture is as described in Section~\ref{section:multitask_unn}.
We run a baseline for each task, where the model is run only for the specific task and the weights are updated for that task only. The idea is to validate our assumption that adding a second task would improve the result of the first task (sentiment classification). When multiple energy updates are executed, the tasks inform one another and we expect to see improvement if the tasks are correlated.

We fine-tune the learning rate and use a value of 0.0001. We also fine-tuned the weight between the two tasks and end up with a weight 0.6 for the sentiment and 0.4 for the genre task.

Table~\ref{table_multitask_results} shows the results from the experiments. We show the average of 5 runs for the UNN. The results show that training both tasks together and having more energy update iterations improves the prediction of the first task (sentiment classification).

\begin{table*}[]
    \centering
    \caption{Results from multitask learning - sentiment and genre classification of IMDB movie reviews. \andre{are these results up-to-date?}}
    \begin{tabular}{c|c|c}
         & Accuracy Sentiment & Accuracy Genre \\
         Baseline Sentiment & 77.63 & \-- \\
         Baseline Genre & \-- & 89.77 \\
         Baseline Both (UNN with k=1) & 79.43 & 88.51 \\
         Both, k=2 & 75.72 & 88.41 \\
         Both, k=3 & \textbf{80.56} & 88.51 \\
         Both, k=4 & 78.75 & 87.48 \\
         Both, k=5 & 79.66 & 88.46 \\
    \end{tabular}
    \label{table:multitask_results}
\end{table*}

\tsvm{TODO: We also make the assumption that in test time, when the gold label for one of the tasks is given, this leads to improving the prediction of the other task. i.e. in this case, when predicting sentiment, we pass the gold label of the genre and expect the multiple updates to lead to improved prediction of the sentiment.}



==> [ICML 2022] Undirected Neural Networks/acknowledgements.tex <==
\section*{Acknowledgements}
We would like to thank M\'ario Figueiredo, Caio Corro and the DeepSPIN team for helpful discussions. TM and AM are supported by the European Research Council (ERC StG DeepSPIN 758969)  %, the P2020 program MAIA (LISBOA-01- 0247- FEDER-045909), 
and by the Fundação para a Ciência e Tecnologia through contracts PTDC/CCI-INF/4703/2021 (PRELUNA) and  UIDB/50008/2020. VN is partially supported by the Hybrid Intelligence Centre, a 10-year programme funded by the Dutch Ministry of Education, Culture and Science through the Netherlands Organisation for Scientific Research (\href{https://hybrid-intelligence-centre.nl/}{https://hybrid-intelligence-centre.nl/}).

==> [ICML 2022] Undirected Neural Networks/appendices.tex <==
\newpage
\appendix
\onecolumn

\section{Proof of \cref{lemma:unrolling}}\label{sec:proof_lemma_unrolling}

We provide a more general proof for multilinear factor potentials, of which  bilinear potentials are a special case. 
Let $\mathcal{G} = (V,F)$ be the factor graph underlying the UNN, with energy function $E(x_1, \ldots, x_n) = \sum_i E_{\var{X}_i}(x_i) + \sum_f E_{f}(x_f)$. We assume $E_{\var{X}_i}(x_i) = -b_i^\top x_i + \Psi_{\var{X}_i}(x_i)$ for each $\var{X}_i \in V$, with $\Psi_{\var{X}_i}$ convex, and $E_{f}(x_f) = -\DP{W_f}{\otimes_{j \in f} x_j}$ for each higher order factor $f \in F$ (multilinear factor energy), 
where $\otimes$ is the outer product, and $W_f$ is a parameter tensor
%in this Kronecker space. 
of matching dimension.
For pairwise factors $f = \{\var{X}_i, \var{X}_j\}$, the factor energy is bilinear and can be written simply as $E_{f}(x_i, x_j) = -x_i^\top W_f x_j$.

The (block) coordinate descent algorithm updates each representation $x_i \in V$ sequentially, leaving the remaining representations fixed. 
Let $F(\var{X}_i) = \{f \in F \,:\, \var{X}_i \in f\} \subseteq F$ denote the set of factors $\var{X}_i$ is linked to. 
The updates can be written as:
\begin{align}
    (x_i)_\star &= \arg\min_{x_i} E_{\var{X}_i}(x_i) + \sum_{f \in F(\var{X}_i)} E_f(x_f)\nonumber\\
    &= \arg\min_{x_i} \Psi_{\var{X}_i}(x_i) \underbrace{-b_i^\top x_i - \sum_{f \in F(\var{X}_i)} \DP{W_f}{\displaystyle\bigotimes_{j \in f} x_j}}_{-z_i^\top x_i}\nonumber\\
    &= (\nabla \Psi_{\var{X}_i}^*)(z_i),
\end{align}
where 
$z_i$ is a pre-activation given by 
\begin{align}
    z_i &= \left(\sum_{f \in F(\var{X}_i)} \rho_i(W_f) \bigotimes_{j \in f, j \ne i} x_j\right) + b_i,
\end{align}
and $\rho_i$ is the linear operator that reshapes and rolls the axis of $W_f$ corresponding to $x_i$ to the first position.  
%and $\nabla \Psi_{\var{X}_i}^*$ is the gradient of the conjugate of the regularizer $\Psi_{\var{X}_i}$.   
If all factors are pairwise, the update is more simply:
\begin{align}
    (x_i)_\star &= (\nabla \Psi_{\var{X}_i}^*)\left(\sum_{f = \{\var{X}_i, \var{X}_j\} \in F(\var{X}_i)} \rho_i(W_f) x_j + b_i\right),
\end{align}
where $\rho_i$ is either the identity or the transpose operator.
The update thus always consists in applying a (generally non-linear) transformation $\nabla \Psi_{\var{X}_i}^*$ to an affine transformation of the neighbors of $\var{X}_i$ in the graph (that is, the variables that co-participate in some factor). 

Therefore, given any topological order of the variable nodes in $V$, running $k$ iterations of the coordinate descent algorithm following that topological order is equivalent to performing forward propagation in an (unrolled) directed acyclic graph, where each node applies affine transformations on input variables followed by the activation function $\nabla \Psi_{\var{X}_i}^*$. 


% \section{Proof of Regularizers to Activation Functions}
% \vlad{Do we want to keep this section? Is it referenced in the body? If yes, the notation is a bit outdated and the writing needs some editing too.} \tsvm{it is not referenced in the body.}

% \andre{one organization possibility is to state this as a more general proposition for an arbitrary pairwise factor graph, where all factor energies are bilinear and all unary energies are linear plus regularized. Then coordinate descent on the energy results in a chain of affine transformations followed by non-linear activations, applied on a particular order, turning this into a traditional computation graph -- ``Unrolling lemma''}
% \vlad{"conjugate gradient" is not the correct term here. Use $*$ vs $\star$ consistently and explain in notation section.}

% We are going to give a proof for one of the functions in \cref{table:unn_functions} -- $\Reg_h(h)  \frac{1}{2}\|h\|^{2} $, in order to give some intuition how these are derived. 

% Let $\Reg_h(h) = \frac{1}{2}\|h\|^{2} $. 
% Then $\Reg_h^{*}(x) = min_{h} \frac{1}{2}\|h\|^{2} - h^{T} t$ and we are looking for the solution $h^\star$. This function is strongly convex, and to find the solution we need to set the gradient to 0. 
% The gradient is $\nabla_h 0.5 ||h||^2 - h^{T} t = h - t = 0$. Then $h^\star = t$.

% Therefore, if we choose as a regularizer the function $\Reg_h(h) = \frac{1}{2}\|h\|^{2} $, the $h^\star(x)$ that minimizes the energy, given $t$, corresponds to the identity activation, $h^\star=t$. 


\section{Analysis of Order and Number of Variable Updates}\label{appendix:order_number_updates}

For one of the experiments - undirected self-attention, we analyze how the order of variable updates and the number of update passes during training affect the model performance. 

\paragraph{Order of variable updates.} 
In \cref{section:experiments_attention} we showed that one pass of the ``forward-backward'' order or variable updates ($\var{Q,K,V,S,H,S,V,K,Q,\hat{X}}$) performs well enough for the of sequence completion. 
Since the flexibility of our model does not limit us to a specific order, we compare it to a random order of updating the variables (a permutation of $\var{Q,K,V,S,H}$; $\var{\hat{X}}$ is always updated last). One pass over the ``forward-backward'' order performs nine variable updates, and one pass over the random order - five. In \cref{fig:attn_update_order_default_vs_random} we show how the two ways of order perform for different number of variable updates (for example, 2 passes over the ``forward-backward'' model equal 18 variable updates, and over the random model - 10). 
The ``forward-backward'' order performs best, but the random order can achieve similar performance after enough number of updates.

% We showed that following the default order of updating the variables, for $k=1$ iteration and zero initialization of the variables, recovers a directed neural network. But the flexibility of our model allows the variables to be updated in any order and no one should be theoretically preferred over the other. Therefore, we experiment what happens when the variables are updated in a random order. \cref{fig:attn_num_updates_comparison} shows learning curves for validation accuracy for different setup. On the first plot -- default order -- shows results for the case where the variables are updated in the default order ($\rightarrow \var{K/Q/V} \rightarrow \var{S} \rightarrow \var{H} \rightarrow \var{V} \rightarrow \var{S} \rightarrow \var{Q/K} \rightarrow \var{X}$). The second plot -- random order fixes the updates of $\var{X}$, i.e. $\var{X}$ is always updated last, but the order of update of the rest of the variables is random. For $k=1$ the model does not learn anything, as most of the variables are zero. But with increasing the number of energy update iterations, the performance is better. The model with random order of variable updates learns slower-- it takes more training steps to achieve the same results as the default order, but it appears to be more stable. The learning rate for the random model is different ($0.00005$).
% \vlad{is it me or the story changes? k=rand is slower in default older, but faster in random order?}\tsvm{Yes, that's right. But the k-s that work for both are different - the default order 'prefers' smaller ks $<3$, while random is better for $>3$.}

\begin{figure}[ht!]
    \centering
    \includegraphics[width=.45\textwidth]{img/attn_default_order.pdf}
    \includegraphics[width=.45\textwidth]{img/attn_random_order.pdf}
    \caption{Learning curves for random number of variable update passes - for ``forward-backward'' and random order of operation updates.}
    \label{fig:attn_num_updates_comparison}
\end{figure}

\paragraph{Number of Energy Update Iterations}

In addition to comparing the number of energy update iterations $k$, we also try setting a random number of updates during training. 
% In \cref{fig:attn_unn_iter_comparison} we show learning curves for validation accuracy for random number of energy update iterations for default and random number of iterations. On training, we choose randomly a number $k \in [1..5]$ and perform this number of updates. The two plots compare the results for inference, where the number of iterations is fixed as $k \in [1, 3, 5]$. 
Instead of specifying a fixed number of iterations $k$, we take a random $k$ between 1 and 5 and train the model with it. We evaluate the performance on inference with $k=3$ (the average value).
In \cref{fig:attn_num_updates_comparison} we compare the performance of the best model trained with random number of iterations $k$ with the best performing models trained with fixed $k$. 
As the plots show, the model trained with a random number of iterations performs on par with the best models with fixed $k$, but takes more time to train.

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=.6\textwidth]{img/attn_default_order_randk.png} 
%     \includegraphics[width=.6\textwidth]{img/attn_random_order_randk.png}
%     \caption{Comparison of learning curves for random number of energy updates updates on training and fixed number of iterations on inference ($k \in [1,3,5]$).}
%     \label{fig:attn_unn_iter_comparison}
% \end{figure}

\section{Analysis of Alternative Initialization Strategies}\label{appendix:alternative_initializations}
In addition to the zero initialization for the output variable $y$, we also experiment with two more initialization strategies - random and uniform initialization. 
We perform this comparison for the MNIST experiment from \cref{section:experiments_mnist}.
For the random initialization, we initialize $y$ with random numbers from a uniform distribution on the interval $[0,1)$
% \vlad{standard normal?} 
and apply $\softmax$. For the uniform initialization, we assign equal values summing to one. 
We compare to the zero initialization strategy on the MNIST forward-backward experiment with $\gamma=.1$.
% \vlad{this makes it sound like random/uniform do not use forward-backward training, don't you mean ``we compare to the zero initialization strategy on the MNIST forward-backward experiment with $\gamma=.1$?}
The results are presented in \cref{tab:alternative_initialization}. 
Random initialization shows promise, but the differences are small, and zero-init has the advantage of clearer parallels to the feed-forward case, so we report that and use it throughout all other experiments. The alternative initialization strategies can be further explored in further work.
% \vlad{In particular say: ``random initialization shows promise'' maybe., and somewhere say that this should be explored in further work?}

\begin{table}[ht]
    \centering
    \caption{Comparison of different initialization strategies for the MNIST experiment from \cref{section:experiments_mnist}.}
    \vskip 0.15in
    \begin{sc}
    \begin{tabular}{cccccc}
        \toprule
         Initialization & $k=1$ & $k=2$ & $k=3$ & $k=4$ & $k=5$ \\
         \midrule
         zero & 98.75 & 98.74 & 98.83 & 98.78 & 98.69 \\
         random & 98.77 & 98.83 & 98.90 & 98.85 & 98.70 \\
         uniform & 98.76 & 98.74 & 98.83 & 98.78 & 98.68 \\
        \bottomrule
    \end{tabular}
    \end{sc}
    \label{tab:alternative_initialization}
\end{table}


\section{Results for forward-only UNN for MNIST}
In addition to the results for forward-backward training of the UNN, we also report results from training the UNN only in forward mode with $\gamma=0$, i.e. when the model is trained for image classification only. The results are in \cref{table:mnist_results_forward_only}. 
% Here more iterations do not generally improve the classification accuracy. 

\begin{table}[h]
    \caption{MNIST accuracy with convolutional UNN in forward-only mode (\ie $\gamma=0$).}
    \vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
    \begin{tabular}{ll}
    \toprule
        Iterations & Accuracy \\
        \midrule
        % $\gamma=0$ & \\
        % \midrule
        $k=1,\gamma=0$ (baseline) & 98.80 \\
        $k=2$ & \textbf{98.82} \\
        $k=3$ & 98.75 \\
        $k=4$ & 98.74 \\
        $k=5$ & 98.69 \\
    \bottomrule
    \end{tabular}
\end{sc}
\end{small}
\end{center}
    \label{table:mnist_results_forward_only}
\end{table}


\section{Additional visualizations}\label{appendix:additional_viz}

% \paragraph{MNIST digit prototypes.}
% \Cref{fig:mnist_generated_full} shows the protoypes induced by an undirected convnet (a,b) and a standard feed-forward one (c) for all classes $0$--$9$.

% \begin{figure}[t]
%     \def\figh{9cm}%
%     \centering
%     \subcaptionbox{}{
%     \includegraphics[height=\figh]{img/undirected_convnet_5iter_full.pdf}}\quad%
%     \subcaptionbox{}{\includegraphics[height=\figh]{img/undirected_convnet_1iter_full.pdf}}\quad%
%     \subcaptionbox{}{\includegraphics[height=\figh]{img/undirected_convnet_1iter_untrained_full.pdf}}%
%     \caption{Digit prototypes generated by convolutional UNN.
% (a) best UNN ($k=5,\alpha=.1)$, (b)
% single iteration UNN ($k=1,\alpha=.1)$,
% (c): standard convnet ($k=1,\alpha=0$). Extended version of \cref{fig:mnist_generated}.\label{fig:mnist_generated_full}}
% \end{figure}

\paragraph{Undirected self-attention weights.}
In \cref{fig:example_attn_weights} we show an example of the weights of the undirected self-attention described in \cref{section:experiments_attention}. The attention weights are the values of the variable $\var{S}$ calculated in the forward and backward pass. 
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.3\textwidth]{img/attn_default_k1_f.pdf}\hfill
    \includegraphics[width=0.3\textwidth]{img/attn_default_k2_iter1_f.pdf}\hfill
    \includegraphics[width=0.3\textwidth]{img/attn_default_k2_iter2_f.pdf}
    \\\medskip
    % another example:
    \includegraphics[width=0.32\textwidth]{img/attn_default_k1_f_ex3.pdf}\hfill
    \includegraphics[width=0.32\textwidth]{img/attn_default_k2_iter1_f_ex3.pdf}\hfill
    \includegraphics[width=0.32\textwidth]{img/attn_default_k2_iter2_f_ex3.pdf}
    % another example:
    \\\medskip
    \includegraphics[width=0.29\textwidth]{img/attn_default_k1_f_ex2.pdf}\hfill
    \includegraphics[width=0.29\textwidth]{img/attn_default_k2_iter1_f_ex2.pdf}\hfill
    \includegraphics[width=0.34\textwidth]{img/attn_default_k2_iter2_f_ex2.pdf}
    \caption{Example of the self-attention weights for models trained with $k=1$ (left) and $k=2$ after one iteration (middle) and two iterations (right). 
    For $k=2$, the model is more like an unrolled two-layer attention mechanism, with the first step identifying an off-diagonal pattern and the latter pooling information into an arbitrary token.
    %The plots show the attention weights for the forward pass, as the plot for the backward pass is almost identical visually.
    }
    \label{fig:example_attn_weights}
\end{figure*}

\paragraph{Dependency tree packed representation}
\Cref{fig:example_marginals} shows an example of how the trees are represented in the output of the model in \cref{section:experiments_parsing}. 

\begin{figure}
    \centering%
\def\H{.5}
\def\W{.9}
\begin{tikzpicture}[
    factoredge/.style={ultra thick,red},
    factor/.style={fill, rectangle, minimum width=2pt, minimum height=2pt},
    bv/.style={font=\small\tt}
    ]
\def\wa{undirected}
\def\wb{neural}
\def\wc{net}
\def\fdr{0}
\def\fdo{1}
\def\fdw{0}
\def\for{0}
\def\fod{0}
\def\fow{1}
\def\fwd{0}
\def\fwo{0}
\def\fwr{1}
\foreach \i in {1,...,3}{
\foreach \j in {1,...,3}{
    \coordinate (var \i-\j) at (\i*\W, \j*\H) {};
}
}
\pgfmathparse{int(40*\fdw)}
\node[bv, fill=red!\pgfmathresult] (dw) at (var 1-1) {\fdw};
\pgfmathparse{int(40*\fdo)}
\node[bv, fill=red!\pgfmathresult] (do) at (var 1-2) {\fdo};
\pgfmathparse{int(40*\fdr)}
\node[bv, fill=red!\pgfmathresult] (dr) at (var 1-3) {\fdr};
\pgfmathparse{int(40*\fow)}
\node[bv, fill=red!\pgfmathresult] (ow) at (var 2-1) {\fow};
\pgfmathparse{int(40*\fod)}
\node[bv, fill=red!\pgfmathresult] (od) at (var 2-3) {\fod};
\pgfmathparse{int(40*\for)}
\node[bv, fill=red!\pgfmathresult] (or) at (var 2-2) {\for};
\pgfmathparse{int(40*\fwo)}
\node[bv, fill=red!\pgfmathresult] (wo) at (var 3-2) {\fwo};
\pgfmathparse{int(40*\fwd)}
\node[bv, fill=red!\pgfmathresult] (wd) at (var 3-3) {\fwd};
\pgfmathparse{int(40*\fwr)}
\node[bv, fill=red!\pgfmathresult] (wr) at (var 3-1) {\fwr};
%\node[left=10pt of var 1-4] {\small\texttt{*}$\to$};
\node[left=10pt of var 1-3] {\small\texttt{\wa}$\to$};
\node[left=10pt of var 1-2] {\small\texttt{\wb}$\to$};
\node[left=10pt of var 1-1] {\small\texttt{\wc}$\to$};
\node[above left=20pt of var 1-3,rotate=-35,anchor=east]{\small\texttt{*}$\to$};
\node[above=10pt of var 1-3,anchor=south west,rotate=42] {\small\strut\texttt{\wa}};
\node[above=10pt of var 2-3,anchor=south west,rotate=42] {\small\strut\texttt{\wb}};
\node[above=10pt of var 3-3,anchor=south west,rotate=42] {\small\strut\texttt{\wc}};
\draw[rounded corners=3pt,thick,draw]
    ([xshift=-3pt,yshift=-3pt]dw.south west) rectangle
    ([xshift=3pt,yshift=3pt]wd.north east);
\end{tikzpicture}%
\begin{tikzpicture}[
    factoredge/.style={ultra thick,red},
    factor/.style={fill, rectangle, minimum width=2pt, minimum height=2pt},
    bv/.style={font=\small\tt}
    ]
\def\wa{undirected}
\def\wb{neural}
\def\wc{net}

\def\fdr{.02}
\def\fdo{.55}
\def\fdw{.43}
\def\for{.08}
\def\fod{.07}
\def\fow{.85}
\def\fwr{.90}
\def\fwd{.07}
\def\fwo{.03}
%\coordinate (var 1 e) at (3.5, 2.5);
%\coordinate (var 2 w) at (5.5, 2.5);
%\coordinate (var 2 e) at (6.5, 2.5);
%\coordinate (var 3 w) at (8.5, 2.5);
\coordinate (var 1 ne);
\foreach \i in {1,...,3}{
\foreach \j in {1,...,3}{
    \coordinate (var \i-\j) at (\i*\W, \j*\H) {};
}
}
\pgfmathparse{int(40*\fdw)}
\node[bv, fill=red!\pgfmathresult] (dw) at (var 1-1) {\fdw};
\pgfmathparse{int(40*\fdo)}
\node[bv, fill=red!\pgfmathresult] (do) at (var 1-2) {\fdo};
\pgfmathparse{int(40*\fdr)}
\node[bv, fill=red!\pgfmathresult] (dr) at (var 1-3) {\fdr};
\pgfmathparse{int(40*\fow)}
\node[bv, fill=red!\pgfmathresult] (ow) at (var 2-1) {\fow};
\pgfmathparse{int(40*\fod)}
\node[bv, fill=red!\pgfmathresult] (od) at (var 2-3) {\fod};
\pgfmathparse{int(40*\for)}
\node[bv, fill=red!\pgfmathresult] (or) at (var 2-2) {\for};
\pgfmathparse{int(40*\fwo)}
\node[bv, fill=red!\pgfmathresult] (wo) at (var 3-2) {\fwo};
\pgfmathparse{int(40*\fwd)}
\node[bv, fill=red!\pgfmathresult] (wd) at (var 3-3) {\fwd};
\pgfmathparse{int(40*\fwr)}
\node[bv, fill=red!\pgfmathresult] (wr) at (var 3-1) {\fwr};
\node[above=10pt of var 1-3,anchor=south west,rotate=42] {\small\strut\texttt{\wa}};
\node[above=10pt of var 2-3,anchor=south west,rotate=42] {\small\strut\texttt{\wb}};
\node[above=10pt of var 3-3,anchor=south west,rotate=42] {\small\strut\texttt{\wc}};
\draw[rounded corners=3pt,thick,draw]
    ([xshift=-3pt,yshift=-3pt]dw.south west) rectangle
    ([xshift=3pt,yshift=3pt]wd.north east);
\end{tikzpicture}
\caption{``Packed'' matrix representation of a dependency tree (left) and dependency arc marginals (right).
Each element corresponds to an arc \texttt{h$\rightarrow$m},
and the diagonal corresponds to the arcs from the root,
\texttt{*$\rightarrow$m}. The marginals, computed via the matrix-tree theorem,
are the structured counterpart of softmax, and correpond to arc probabilities.
% \vlad{This might be well suited to moving to supp?}
}
\label{fig:example_marginals}
\end{figure}

\section{Derivation of updates for convolutional UNN}
\label{section:conv_derivation}
The two-layer convolutional UNN is defined by the pairwise energies
\begin{equation}
\begin{aligned}
E_\var{XH_1}(X, H_1) &= -\DP{H_1}{\mathcal{C}_1(X; W_1)} \,, \\
E_\var{H_1H_2}(H_1, H_2) &= -\DP{H_2}{\mathcal{C}_2(H_1; W_2)}\,,\\
E_\var{H_2Y}(H_2, y) = -\DP{y}{VH_2}\,,
\end{aligned}
\end{equation}
and the unary energies
\begin{equation}
\begin{aligned}
E_\var{X}(X) &= \frac{1}{2}\|X\|_2^2 \,, \\
E_\var{H_1}(H_1) &= -\DP{H_1}{b_1 \otimes 1_{d_1}} + \Psi_{\tanh}(H_1)\,, \\
E_\var{H_2}(H_2) &= -\DP{H_2}{b_2 \otimes 1_{d_2}} + \Psi_{\tanh}(H_2)\,, \\
E_\var{Y}(y) &= -\DP{b}{y} - \entropy(y) \,. \\
\end{aligned}
\end{equation}
Above, $\mathcal{C}_1$ and $\mathcal{C}_2$ are 
are linear cross-correlation (convolution) operators with
stride two and filter weights $W_1 \in \reals^{32 \times 1 \times 6 \times 6}$ and $W_2 \in \reals^{64 \times 32 \times 4 \times 4}$, and
$b_1 \in \reals^{32}$ and $b_2 \in \reals^{64}$ are vectors of
biases for each convolutional filter. The hidden activations have dimension
$H_1 \in \reals^{32 \times (d_1)}$
and
$H_2 \in \reals^{64 \times (d_2)}$,
where $d_1$ and $d_2$ are tuples that depend on the input image size; for MNIST, $X \in \reals^{1 \times 28 \times 28}$ leading to $d_1=12 \times 12$ and $d_2=5 \times 5$.

To derive the energy updates, we use the fact that a real linear operator $\mathcal{A}$ interacts with the Frobenius inner product as:
%\mathcal{C}$ is a linear operator and therefore interacts 
\begin{equation}
\DP{P}{\mathcal{A}(Q)} = \DP{Q}{\mathcal{A}^\top(P)}\,,
\end{equation}
where $\mathcal{A}^\top$ is the transpose, or adjoint, operator.\footnote{This generalizes the observation that $p^\top A q = q^\top A^\top p$.}
If $\mathcal{C}$ is a convolution (\ie, \verb|torch.conv2d|)
then $\mathcal{C}^\top$ is a deconvolution (\ie, \verb|torch.conv_transpose2d|) with the same filters.
We then have
\begin{equation}
\begin{aligned}
E_\var{XH_1}(X, H_1) &= -\DP{H_1}{\mathcal{C}_1(X; W_1)} 
=-\DP{X}{\mathcal{C}_1^\top(H_1; W_1)} \,, \\
E_\var{H_1H_2}(H_1, H_2) &= -\DP{H_2}{\mathcal{C}_2(H_1; W_2)}
=-\DP{H_1}{\mathcal{C}_2^\top(H_2; W_2)}\,.\\
\end{aligned}
\end{equation}
Adding up all energies and ignoring the constant terms in each update, we get
\begin{equation}
\begin{aligned}
X_\star &= \argmin_X -\DP{X}{\mathcal{C}_1^\top(H_1, W_1)} + \Psi_{\tanh}(X) \\
&= \tanh(\mathcal{C}_1^\top(H_1, W_1))\,, \\
(H_1)_\star &= \argmin_{H_1} 
-\DP{H_1}{\mathcal{C}_1(X, W_1)} 
-\DP{H_1}{\mathcal{C}_2^\top(H_2, W_2)} 
-\DP{H_1}{b_1 \otimes 1_{d_1 \times d_1}}
+ \Psi_{\tanh(H_1)} \\
&= \tanh(
\mathcal{C}_1(X, W_1)+
\mathcal{C}_2^\top(H_2, W_2)+
b_1 \otimes 1_{d_1 \times d_1}
)\,, \\
(H_2)_\star &= \argmin_{H_2} 
-\DP{H_2}{\mathcal{C}_2(H_1, W_2)} 
-\DP{H_2}{\sigma_y(V)y}
-\DP{H_2}{b_2 \otimes 1_{d_2 \times d_2}}
+ \Psi_{\tanh(H_2)} \\
&= \tanh(
\mathcal{C}_2(H_1, W_2)
+\sigma_y(V)y
+b_2 \otimes 1_{d_2 \times d_2}
)\,, \\
y_\star &=
-\DP{y}{V H_2} - \DP{y}{b} - \entropy{y} \\
&= \softmax(VH_2 + b)\,.
\end{aligned}
\end{equation}
Note that in our case,
$H_2 \in \reals^{64 \times 5 \times 5}$,
$V \in \reals^{10 \times 64 \times 5 \times 5}$ and
thus $VH_2 \in \reals^{10}$ is a tensor contraction (\eg, \verb|torch.tensordot(V, H_2, dims=3)|).
The $\sigma_y$ linear operator -- opposite of $\rho$ from \cref{lemma:unrolling} -- rolls the axis of $V$ corresponding to $y$ to the \emph{last} position, such that
$\sigma_y(V) \in \reals^{64 \times 5 \times 5 \times 10}$, the tensor analogue of a transposition (\eg, \verb|torch.permute(V, (1, 2, 3, 0))|.)


==> [ICML 2022] Undirected Neural Networks/background.tex <==
% Energy-Based Models capture dependencies by associating a scalar energy (a measure of compatibility) to each configuration of the variables in a model. 
% Inference, i.e., making a prediction or decision, consists in setting the value of observed variables and finding values of the remaining variables that minimize the energy. Learning consists in finding an energy function that associates low energies to correct values of the remaining variables, and higher energies to incorrect values. A loss function, minimized during learning, is used to measure the quality of the available energy functions \citep{lecun2006tutorial}.

% Let us consider a model with two sets of variables, $x$ and $y$. Following the examples of NLI \andre{not defined so far. consider replacing by a different example in case we don't do NLI in the paper}, variable $x$ could be a representation of the premise and hypothesis. Variable $y$ could be a discrete variable that represents the possible category of the object. For example, in the NLI case $y$ could take three possible values: entailment, contradiction, neutral. The model is viewed as an energy function which
% measures how good each configuration of $x$ and $y$ is. The output number (i.e. the energy) can be interpreted as a measure of how much $x$ and $y$ are compatible. 

% Small energy would mean that the variables are highly compatible and vice versa.  The energy function is denoted as $E(x,y)$.

% In the energy-based model, the input $x$ is given (observed), and the model produces the $y$ that is most compatible with the observed $x$ \citep{lecun2006tutorial}. 
% As a result, we would like to find $y^{*}$
% , chosen from a set $Y$, for which
% $E(x,y)$ is the smallest:
% $y^{*} = \argmin_{y} E(x,y)$ \andre{I think we can keep only this paragraph and delete the previous two. Maybe rephrase as ``An energy-based model is a network which takes as inputs $x$ (observed) and $y$ (a candidate output from a set $\mathcal{Y}$) and computes an energy function $E_\theta(x,y)$, which defines the compatibility between $x$ and $y$. The goal is to the predict $y^{*} \in \mathcal{Y}$ that minimizes the energy, $y^{*} = \argmin_{y} E_\theta(x,y)$. This corresponds to the most probable output under a Gibbs distribution, $p_\theta(y \mid x) \propto \exp(-E_\theta(x,y))$, avoiding modeling this distribution explicitly.''}

An energy-based model is a network which takes as inputs $x$ (observed) and $y$ (a candidate output from a set $\mathcal{Y}$) and computes an energy function $E_\theta(x,y)$, which defines the compatibility between $x$ and $y$. The goal is to the predict $y^{*} \in \mathcal{Y}$ that minimizes the energy, $y^{*} = \argmin_{y} E_\theta(x,y)$. This corresponds to the most probable output under a Gibbs distribution, $p_\theta(y \mid x) \propto \exp(-E_\theta(x,y))$, avoiding modeling this distribution explicitly.

\subsection{Hopfield Networks}
% \andre{This subsection can be trimmed a bit and potentially moved to the related work section, unless it makes it easier for us to explain our UNNs. Also this definitions are not distinguishing between Hopfield and Boltzmann networks, right?}
Hopfield networks \citep{hopfield1982neural} consist of binary units with symmetric, bidirectional connection weights between them, i.e. each unit is connected to all other units \citep{stone2019artificial}. The total input to a unit depends on the states of all other units.
The energy function is  defined for every possible set of unit states and the total energy is the sum of the energies of all units.

% The energy function is  defined for every possible set of unit states by the formula:

% \begin{equation}
%     E(y) = -\sum_{i=1}^{K}\sum_{j=i+1}^{K}w_{ij}y_{i}y_{j}
% \end{equation}

% where $w$ are the weights, $y$ are the states of the units and $K$ is the number of units.

% The energy contributed by a single unit is:

% \begin{equation}
%     E_{i} = -y_{i}\sum_{j=1}^{K}w_{ij}y_{j}
% \end{equation}

% And the total energy is the sum of the energies of all units:

% \begin{equation}
%     E(y) = \sum_{i=1}^{K}E_{i}
% \end{equation}

% The energy function is derived  from statistical mechanics, where it is called the Hamiltonian; in  optimisation theory it is called a Lyapunov function \citep{stone2019artificial}.

% The continuous Hopfield networks \citep{hopfield1984neurons} 

% Recent work \citep{ramsauer2020hopfield} shows that the attention mechanism of the widely used Transformer model \citep{vaswani2017attention} is equal to the update rule of a Hopfield network with continuous states \citep{hopfield1984neurons}. 


\subsection{Boltzmann Machines}

% \andre{this section can also be trimmed, we don't need to have special subsections for RBMs and DBMs and write all the equations, we only need to mention them briefly.} 
A Boltzmann Machine \citep{ackley1985learning} is a network of symmetrically connected, neuronlike units that make stochastic decisions about whether to be on or off. Boltzmann machines have a simple learning algorithm that allows them to discover
interesting features in datasets composed of binary vectors. The learning algorithm is intractable in networks with many layers of features. \citep{hinton2007boltzmann}
% detectors, but it can be made much faster by learning one layer of  feature detectors at a time. \citep{hinton2007boltzmann}

% Boltzmann machines are pairwise fully connected neural
% networks with N visible units $x \in \{0, 1\}^{N}$ and M hidden units $x \in \{0, 1\}^{M}$.
% They define the following energy function:

% \begin{equation}
% E(x, h) = -x^{T}Rx - h^{T}Wx - h^{T}Sh - a^{T}x - b^{T}h
% \end{equation}

% The probability of a configuration is defined as:

% \begin{equation}
% P(x, h) = \frac{\exp(-E(x, h))}{Z}
% \end{equation}

% \noindent(where Z is the partition function)
% and maximizing the probability corresponds to minimizing the energy. We can represent a Boltzmann machine with the factor graph diagram in Figure 1, defining a bilinear factor energy

% \begin{equation}
%     E_{x, h}(x, h) = - h^{T}Wx
% \end{equation}

% \noindent and unary energies

% \begin{equation}
%     E_{x}(x) = - x^{T}Rx- a^{T}x + \iota_{\{0,1\}^{N}}(x)
% \end{equation}

% \noindent and 

% \begin{equation}
%     E_{h}(h) = - h^{T}Wx - b^{T}h + \iota_{\{0,1\}^{M}}(h)
% \end{equation}

% \noindent $\iota_{\{0,1\}^{N}}(x)$ means that we set constraints for $x$ to be a binary vector with $N$ units.
% \vlad{define this more clearly in the notations section}


% \subsection{Restricted Boltzmann Machines} 
% Restricted Boltzmann machines are special cases of Boltzmann machines where the connections between visible and hidden units form a bipartite graph. In this case, we have:

% \begin{equation}
%     E_{X, H}(x, h) = - h^{T}Wx
% \end{equation}

% \begin{equation}
%     E_{X}(x) = - a^{T}x + \iota_{\{0,1\}^{N}}(x)
% \end{equation}

% \begin{equation}
%     E_{H}(h) = - b^{T}h + \iota_{\{0,1\}^{M}}(h)
% \end{equation}


% \subsection{Deep Boltzmann Machines} 
% Deep Boltzmann machines are similar to restricted Boltzmann machines, but
% with more layers. Here we have:

% \begin{equation}
%     E_{X, H_{1}}(x, h_{1}) = - h_{1}^{T}W_{1}x
% \end{equation}

% \begin{equation}
%     E_{H_{k-1}, H_{k}}(h_{k-1}, h_{k}) = - h_{k}^{T}W_{k}x
% \end{equation}

% \begin{equation}
%     E_{X}(x) = - a^{T}x + \iota_{\{0,1\}^{N}}(x)
% \end{equation}

% \begin{equation}
%     E_{H_{k}}(h_{k}) = - b_{k}^{T}h_{k} + \iota_{\{0,1\}^{M_{h}}}(h_{k})
% \end{equation}



The Boltzmann Machines are pairwise fully connected neural networks with $N$ visible units $x$ and $M$ hidden units $h$. The probability of a configuration is defined as: 

\begin{equation}
    P(x,h) = \frac{exp(-E(x,h))}{Z}
\end{equation}

Maximizing the probability corresponds to minimizing the energy.

\begin{equation}
    E(x,h) = - x^{T}Rx - h^{T}Wx - h^{T}Sh - a^{T}x - b^{T}h
\end{equation}

The total energy is given by:

\begin{equation}
    E(x,h) = E_{X}(x) + E_{H}(h) + E_{X,H}(x,h)
\end{equation}

where

\begin{equation}
    E_{X,H}(x,h) = - h^{T}Wx
\end{equation}

\begin{equation}
    E_{X}(x) = - a^{T}x + \iota_{\{0,1\}^{N}}(x)
\end{equation}

\begin{equation}
    E_{H}(h) = - b^{T}h + \iota_{\{0,1\}^{M}}(h)
\end{equation}

where $\iota_{\{0,1\}^{N}}(x)$ means constraint on $x$, i.e. $x$ needs to be $N$ zeros or ones.
% \vlad{define this more clearly in the notations section}


\textbf{Restricted Boltzmann Machines (RBMs)} are special cases of Boltzmann machines where the connections between visible and hidden units form a bipartite graph. \noindent The separation of visible and hidden units in the RBMs allows for more efficient training algorithms than for the general Boltzmann machines \citep{smolensky1986information,hinton2007boltzmann}. 
\textbf{Deep Boltzmann Machines (DBMs)} are similar to restricted Boltzmann machines, but with more layers.

==> [ICML 2022] Undirected Neural Networks/conclusions.tex <==
\section{Conclusions and Future Work}

We presented UNNs -- a structured energy-based model which combines the power of factor graphs and neural networks. At inference time, the model energy is minimized with a coordinate descent algorithm, allowing reuse of existing building blocks in a modular way with guarantees of decreasing the energy at each step. 
We showed how the proposed UNNs subsume many existing architectures, conveniently combining supervised and unsupervised/self-supervised learning, as demonstrated on the three tasks.

We hope our first steps in this work will spark multiple directions of future work on undirected networks. One promising direction is on probabilistic UNNs with Gibbs sampling, which have the potential to bring our modular architectures to  generative models.
Another direction is to consider alternate training strategies for UNNs.
Our strategy of converting UNNs to unrolled neural networks, enabled by \cref{lemma:unrolling}, 
makes gradient-based training easy  to implement,
but alternate training strategies, perhaps based on equilibrium conditions or dual decomposition, hold promise. 
Promising directions could be using this framework for dealing with missing data or learning the joint probability distribution.
%of the training objective. \andre{maybe mention a second idea, briefly}\vlad{how about dual decomposition? does this need more words or is it clear?}

% For future work, one of the possible directions is to invent a better way of training the UNNs, since the current training is actually done as an unrolled directed network 
% \andre{this sentence should be improved. it makes out current approach sound not good enough. perhaps ``Even though our strategy of converting UNNs to unrolled neural networks to train them, enabled by Lemma 1, is convenient, better training strategies for UNNs might exist. As future work, we plan to explore alternate ways of training UNNs}. We would like to explore learning specific to UNNs.
% There is also room for more exploration of UNN-specific details, for example whether and how the order of variable updates matters. 
% Another issue we encountered during the experiments was that when the number of iterations during training and inference differs, the networks does not perform well \andre{I don't think this was reported in the experiments. We should probably not mention that here as it would sound ackward.}. 
% We would like to explore whether random number of iterations during training leads to better performance. \tsvm{We are actually experimenting with this, it was added after writing this paragraph. It's in Appendix C.}


% Hopeful other contributions:

% \begin{itemize}
%     \item Advantages/disadvantages wrt to SPENs for the structured factors case (easier inference and training?)
%     \item Relation with implicit layers (do UNN subsume them?)
%     \item UNNs very general and subsume other frameworks (incl. FFNNs and SPENs)
%     \item generate x given y (eg for mnist)
%     \\ \quad (rel to Grathwohl EBM)
%     \\ \quad (pitch as prototype rather than sampler)
%     \\ \quad (make stochastic?)
% \end{itemize}

==> [ICML 2022] Undirected Neural Networks/experiments_attention.tex <==
\section{Undirected Attention Mechanism}\label{section:experiments_attention}

Attention \citep{bahdanau2014neural,vaswani2017attention} is a key component that enables neural networks to handle variable-length sequences as input.
In this section, we propose an undirected attention mechanism
%The architecture of self-attention is shown on
(\cref{fig:factors_all_models}(e)). We demonstrate this model on the task of completing missing values in a sequence of dynamic length $n$,
with the variable $\var{X}$ serving as both input and output, taking values $X \in
\reals^{d \times n}$, queries, keys and values taking values $Q, K, V \in
\reals^{n \times d}$, and attention weights $S \in (\triangle_n)^n$,
where $d$ is a fixed hidden layer size.
Finally, $\var{H}$ is an induced latent sequence representation, with values $H
\in \reals^{n \times d}$. The only trainable parameters are $W_\var{Q},
W_\var{K}, W_\var{V} \in \reals^{d \times d}$, and the input embeddings.
We model scaled dot-product attention given with
$\softmax(d^{-\frac{1}{2}}QK^\top)V$.
For all variables except $\var{S}$, we set $\energyltwo{\cdot}$. For the attention weights, we use $E_\var{S}(S) = -\sqrt{d}\sum_{i=1}^n \entropy(S_i)$.
%\andre{no biases?}  \vlad{like in parsing, no biases, because the size of S varies}
The higher-order energies are:
\begin{equation}
\begin{aligned}
%    E_\var{XZ}(X,V) &= -\DP{Z}{W_\var{Z}(X+P)}\,,
%    \qquad\text{for}~\var{Z} \in \{\var{V},\var{Q},\var{K}\}\,,\\
    E_\var{XQ}(X,Q) &= -\DP{Q}{W_\var{Q}(X+P)}\,,\\
    E_\var{XK}(X,K) &= -\DP{K}{W_\var{K}(X+P)}\,,\\
    E_\var{XV}(X,V) &= -\DP{V}{W_\var{V}(X+P)}\,,\\
    E_\var{QKS}(Q,K,S) &= -\DP{S}{Q K^\top}\,, %+ \sqrt{d} \textstyle\sum_i \entropy(S_i)\,,
    \\
    E_\var{VSH}(V,S,H) &= -\DP{H}{S V}\,,
\end{aligned}
\end{equation}
where $P$ is a matrix of sine and cosine positional embeddings of same dimensions as $X$ \cite{vaswani2017attention}.

%The updates then become:
Minimizing the energy yields the blockwise updates:
\begin{equation}
\begin{aligned}
    \nextit{Q} &= W_\var{Z}(\currit{X} + P) + S\currit{K}\,, \\
    \nextit{K} &= W_\var{K}(\currit{X} + P) + S^\top {Q}\,, \\
    \nextit{V} &= W_\var{V}(\currit{X} + P) + S^\top \currit{H}\,, \\
    \nextit{S} &= \softmax\left(d^{-1/2}({Q}{K}^\top + {V}{H}^{\top})\right)\,, \\
    \nextit{H} &= {S}{V}\,,\\
    \nextit{\bar{X}} &= {\bar{V}} W_\var{V} + {\bar{Q}} W_\var{Q} +
{\bar{K}} W_\var{K},
\end{aligned}
\end{equation}
where $\bar{X}$ denotes only the rows of $X$ corresponding to the masked
(missing) entries.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{img/attn_default_k1_b.pdf}
    \caption{Undirected self-attention (one ``forward-backward'' pass) identifies an off-diagonal pattern, allowing generalization.
    % \vlad{increase axis label font size, perhaps add colorbar.}
    }
    \label{fig:attn_example_small}
\end{figure}


Provided zero initialization, updating in the order $\var{(V/Q/K),S,H}$
corresponds exactly to a forward pass in a standard self-attention.
However, in an UNN, our expressions allow backward propagation back toward $\var{X}$, as well as iterating to an equilibrium.
To ensure that one round of updates propagates information through all the variables, we employ the ``forward-backward'' order
$\var{Q, K, V, S, H, S, V, K, Q, \bar{X}}$.
% , updating $\bar{\var{X}}$ at the end of each round.

%The default order of updating the variables is in forward from $\var{X}$ to $\var{H}$ and then backward to $\bar{X}$ ($\rightarrow \var{K/Q/V} \rightarrow \var{S} \rightarrow \var{H} \rightarrow \var{V} \rightarrow \var{S} \rightarrow \var{Q/K} \rightarrow \var{X}$).

% \andre{compare here to the regular attention updates?}
% \vlad{These so far are identical to the attention updates but something is missing, S is updated twice, once in forward and once in backward. We need to clarify}
% \tsvm{In the appendix, we have ($\rightarrow K/Q/V \rightarrow S \rightarrow H \rightarrow V \rightarrow S \rightarrow Q/K \rightarrow X$), where we explain the default order and then the random one. Should we add this here?}


We evaluate the performance of the undirected attention with a toy task of sequence completion. We generate a toy dataset of numerical sequences between $1$ and $64$, of length at least 8 and at most 25, in either ascending or descending consecutive order. We mask out up to 10\% of the tokens and generate all possible sequences, splitting them into training and test sets with around 706K and 78K instances. %
% \vlad{describe dataset train/test sizes, overlap.}
%Positional embeddings are added to the input.
Undirected self-attention is applied to the input sequence.
%One update consists of 1) updating the variables $\var{Q}, \var{K}, V$ from the input $X$, 2) updating $S$ and $H$, 3) from them the queries, keys and values are updated again and 4) the input $X$ is updated again.
Note that because of the flexibility of the architecture, the update of the input variable $X$ does not differ from the updates of the remaining variables,
% \vlad{differ than -> differ from?}
because each variable update corresponds to one step of coordinate descent.
%and for the model it does not matter whether the variable is for input, output or hidden.
The model incurs a cross-entropy loss for the missing elements of the sequence and the parameters are updated using Adam with learning rate $10^{-4}$. The hidden dimension is $d=256$, and
gradients with magnitude beyond $10$ are clipped.
%(unrolling of the graph is shown on Section~\ref{section:unn}).

Undirected attention is able to solve this task, reaching over 99.8\% test accuracy, confirming 
%the concept of building attention with our model is 
viablity. \Cref{fig:attn_example_small} shows the attention weights for a model trained with $k=1$. More attention plots are shown in \cref{appendix:additional_viz}.

 % \vlad{test accuracy? might want to describe train/test sets here}
\paragraph{Impact of update order.}
The ``forward-backward'' order is not the only possible order of updates in an UNN.
In \cref{fig:attn_update_order_default_vs_random} we compare its performance against a randomized coordinate descent strategy, where at each round we pick a permutation of $\var{Q,K,V,S,H}$. In both cases, $\var{\bar{X}}$ is updated at the end of each iteration.
(Note that the ``forward-backward'' order performs almost twice the number of updates per iteration.)
While the ``forward-backward'' order performs well even with a single pass, given sufficient iterations, random order updates can reach the same performance, suggesting
that hand-crafting a meaningful order helps but is not necessary.
Further analysis is reported in \cref{appendix:order_number_updates}.

\begin{figure}
    \centering
    \includegraphics[width=.99\linewidth]{img/random_updates.pdf}
    \caption{Comparison of the test accuracy) for models
with random and ``forward-backward'' order of variable updates. 
Markers indicate one full iteration.
%For one pass of the random order, five variable updates are performed, while in the ``forward-backward'' they are nine.
% \vlad{can you get the data here rather than a screenshot from wands and biases? Reviewers can tell.}\tsvm{I think I can get it from wandb, will put a different chart.} \andre{consider moving this fig to supp if we need to save space}
% \vlad{This caption no longer accurate}
}
\label{fig:attn_update_order_default_vs_random}
\end{figure}


==> [ICML 2022] Undirected Neural Networks/experiments_mnist.tex <==
\section{Image Classification and Visualization}\label{section:experiments_mnist}


% \andre{maybe move this section before the undirected attention?}
Unlike feed-forward networks, where the processing order is hard-coded from
inputs $\var{X}$ to outputs $\var{Y}$, UNNs support processing in any
direction. We can thus use the same trained network both for classification as well as for generating prototypical examples for each class.
We demonstrate this on the MNIST dataset of handwritten digits \citep{deng2012mnist},
showcasing convolutional UNN layers.

%\begin{table}
%\texttt{Conv2d(in\_channels=1, out\_channels=32, kernel\_size=6, stride=1)} \\
%\texttt{Conv2d(in\_channels=32, out\_channels=64, kernel\_size=4, stride=1)} \\
%\texttt{Conv2d(in\_channels=32, out\_channels=10, kernel\_size=5, stride=1)} \\
%\texttt{Conv2d(in\_channels=32, out\_channels=64, kernel\_size=4, stride=1)} \\

The architecture is shown in \cref{fig:factors_all_models}(c)
and has the following variables: the image $\var{X}$, the class label
$\var{Y}$ and two hidden layer variables $\var{H}_{\{1,2\}}$.
Unlike the previous examples, the two pairwise energies involving the image and
the hidden layers are convolutional, \ie, linear layers with internal structure:
\begin{equation}
\begin{aligned}
E_\var{XH_1}(X, H_1) &= -\DP{H_1}{\mathcal{C}_1(X; W_1)} \,, \\
E_\var{H_1H_2}(H_1, H_2) &= -\DP{H_2}{\mathcal{C}_2(H_1; W_2)}\,,
\end{aligned}
\end{equation}
where $\mathcal{C}_{1,2}$ are linear cross-correlation operators with
stride two and
filter weights $W_1 \in \reals^{32 \times 1 \times 6 \times 6}$
and
$W_2 \in \reals^{64 \times 32 \times 4 \times 4}$.
The last layer is fully connected:
\begin{equation}
E_\var{H_2Y}(H_2, y) = -\DP{V}{~y~\otimes H_2}\,.
\end{equation}
The unary energies for the hidden layers contain standard (convolutional) 
bias term along with the binary entropy term $\Psi_\text{tanh}(H)$ such that $\nabla
\Psi_\text{tanh}^*(t)=\operatorname{tanh}(t)$ (see \cref{table:unn_functions}).
Note that $\var{X}$ is no longer a constant when generating $\var{X}$ given $\var{Y}$, therefore it is important to specify the unary energy $E_\var{X}$.
Since pixel values are bounded, we set $\var{E}_X(x) = \Psi_\text{tanh}(x)$.
%This factor graph here is similar to the examples (a) and (b) with one more hidden variable, but here we have convolutional and not linear layers.
Initializing $H_1,H_2,$ and $y$ with zeroes and updating them once blockwise in
this order yields exactly a feed-forward convolutional neural network.
As our network is undirected, we may propagate information in multiple passes,
proceeding in the order $\var{H_1, H_2, Y, H_2}$ iteratively.
The
update for $H_1$ involves a convolution of $X$ and a deconvolution
of $H_2$; we defer the other updates to
\cref{section:conv_derivation}:
\begin{equation}
\nextit{(H_1)}\!\!\!\!\!=\operatorname{tanh}(\mathcal{C}_1(\currit{X}; W_1) +
\mathcal{C}^\top_2(\currit{H_2}; W_2) +
b_1 \otimes 1_{d_1})\,,
\end{equation}
where $b_1 \in \reals^{32}$ are biases for each filter,
%applied identically at each location,
and $d_1 = 12 \times 12$ is the convolved image size.
To generate digit prototype $X$ from a given class $c\in\{1,\ldots,10\}$, we may
set $y=e_c$, initialize the other variables at zero (including $\var{X}$),
and solve $\hat{X}=\argmin_X \min_{H_{1,2}} E(X, H_1, H_2, y)$ by coordinate descent in the reverse order $\var{H_2},\var{H_1},\var{X},\var{H_1}$ iteratively.

We train our model jointly for both tasks. For each labeled pair $(X,y)$ from
the training data, we first predict $\hat{y}$ given $X$, then separately predict $\hat{X}$
given $y$.
%in both cases restarting from a zero initialization of all unobserved variables.
The incurred loss is a weighted combination
$\ell(x,y) = \ell_f(y, \hat{y}) + \gamma \ell_b(X, \hat{X})$,
where $\ell_f$ is a 10-class cross-entropy loss,
and $\ell_b$ is a binary cross-entropy loss averaged over all $28\times28$
pixels of the image.
We use $\gamma=.1$ and an Adam learning rate of $.0005$.

\begin{table}[t]
    \caption{MNIST accuracy with convolutional UNN.}
    \vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
    \begin{tabular}{ll}
    \toprule
        Iterations & Accuracy \\
        \midrule
        $k=1,\gamma=0$ (baseline) & 98.80 \\
        $k=1$ & 98.75 \\
        $k=2$ & 98.74 \\
        $k=3$ & \textbf{98.83} \\
        $k=4$ & 98.78 \\
        $k=5$ & 98.69 \\
    \bottomrule
    \end{tabular}
\end{sc}
\end{small}
\end{center}
    \label{table:mnist_results}
\end{table}

%We evaluate two tasks - image classification and image prototype generation. The training happens in two passes. In the standard, forward path, the image is passed to the input and a class is predicted on the output $Y$. At the same time we train the "backward" pass - where the class is passed and the model generates the image prototype, described in Algorithm\ref{alg:fw_bw}.

%\begin{algorithm}
%\begin{algorithmic}
%\label{alg:fw_bw}
%\STATE Sample$(x, y)$ from the dataset
%\STATE Run model in forward mode given $x$, predict $\hat{y}$
%\STATE Incur $loss_{fw}(\hat{y}, y)$
%\STATE Run model in backward mode given $y$, predict $\hat{x}$
%\STATE Incur $loss_{bw}(\hat{x}, x)$
%\STATE $loss = loss_{fw} + w*loss_{bw}$
%\STATE Do gradient update on $loss$
%\caption{Forward and backward pass for image classification and prototype generation.}
%\end{algorithmic}
%\end{algorithm}

%The variables updates are as follows \tsvm{I don't know how the conv energies look like. The variable updates below are form the code, please correct if wrong.}:

%\begin{align*}
    %X = \conv^\top(H_1, W_1) \\
    %H_1 = \conv(H, W_1) +\conv^\top(H_2, W_2) \\
    %H_2 = \conv(H_1, W_2) +Y W_3 \\
    %Y = H_2 W_3^\top
%\end{align*}

The classification results are shown in \cref{table:mnist_results}. The model is able to achieve high classification accuracy, and multiple iterations lead to a slight improvement. This result suggests
the reconstruction loss for $\var{X}$ can also be seen as a regularizer,
as the same model weights are used in both directions.
The more interesting impact of multiple energy updates is the image prototype generation.
In \cref{fig:mnist_generated} we show the generated digit prototypes after several iterations of energy minimization, as well as for models with a single iteration.
The networks trained as UNNs produce recognizable digits, and in particular the model with more iterations learns to use the additional computation to produce clearer pictures.
As for the baseline, we may interpret it as an UNN and apply the same process to extract prototypes, but this does not result in meaningful digits (\cref{fig:mnist_generated}c). 
Note that our model is not a generative model – in that experiment, we are not sampling an image according to a probability distribution, rather we are using energy minimization deterministically to pick a prototype of a digit given its class.

% \vlad{some points to make:
% \begin{itemize}
% \item this experiment demonstrates conv layers and deeper nets
% \item the $x$ reconstruction loss probably has some slight regularization
% potential we might explore further.
% \end{itemize}
% }

\begin{figure}[t]
    \def\figh{9cm}%
    \centering
    \subcaptionbox{}{
    \includegraphics[height=\figh]{img/undirected_convnet_5iter_full.pdf}}\quad%
    \subcaptionbox{}{\includegraphics[height=\figh]{img/undirected_convnet_1iter_full.pdf}}\quad%
    \subcaptionbox{}{\includegraphics[height=\figh]{img/undirected_convnet_1iter_untrained_full.pdf}}%
    \caption{Digit prototypes generated by convolutional UNN.
(a) best UNN ($k=5,\gamma=.1)$, (b)
single iteration UNN ($k=1,\gamma=.1)$,
(c): standard convnet ($k=1,\gamma=0$).
\label{fig:mnist_generated}}
\end{figure}

\paragraph{Comparison of UNN to Unconstrained Model}
As per \cref{fig:unroll_undirected_mlp}, an unrolled UNN can be seen as a feed-forward network with a specific architecture and with weight tying. To confirm the benefit of the UNN framework, we compare against an unconstrained model, \ie, with the same architecture but separate, untied weights for each unrolled layer.
We use as a base the model described in forward-only mode and train a model with 2 to 5 layers with different weights instead of shared weights as in the case with the UNN. Depending on the number of layers, we cut the number of parameters in each layer, in order to obtain models with the same number of parameters as the UNN for fair comparison. The results from the experiment are described in \cref{tab:unconstrained}.

\begin{table}[ht]
    \centering
    \small
    \caption{Comparison of UNN with an unconstrained model with the same number of layers as the UNN iterations. The number of parameters of the UNN and the unconstrained model are roughtly the same.}
    \vskip 0.15in
    \begin{sc}
    \begin{tabular}{cccccc}
        \toprule
          & $k=1$ & $k=2$ & $k=3$ & $k=4$ & $k=5$ \\
         \midrule
        %  UNN & 98.80 & 98.82 & 98.75 & 98.74 & 98.69 \\
        %  \midrule
         Acc. & 98.80 & 98.76 & 98.45 & 98.32 & 97.39 \\
         \midrule
         \# params & 50026 & 51220 & 51651 & 53608 & 51750 \\
        \bottomrule
    \end{tabular}
    \end{sc}
    \label{tab:unconstrained}
\end{table}


==> [ICML 2022] Undirected Neural Networks/experiments_parsing.tex <==
\section{Structured UNNs for Dependency Parsing}\label{section:experiments_parsing}

The concept of UNN can be applied to structured tasks -- all we need to do is to define \textit{structured factors}, as shown next.

We experiment with a challenging structured prediction task from natural language processing: unlabeled, non-projective dependency parsing \citep{kubler2009dependency}.
% \andre{should we have a figure with a dependency tree -- e.g. one where out model gets the full modifier structure and the baseline doesn't -- and point to it here to illustrate the task that we are tackling?} \tsvm{working on it.}
Given a sentence with $n$ words, represented as a matrix $X \in \reals^{r \times n}$ (where $r$ is the embedding size), the goal is to predict the syntactic relations as a \textit{dependency tree}, \textit{i.e.}, a spanning tree which has the words as nodes. The output can be represented as a binary matrix  $Y \in \reals^{n \times n}$, where the $(i,j)\textsuperscript{th}$ entry indicates if there is a directed arc $i \rightarrow j$ connecting the $i\textsuperscript{th}$ word (the \textit{head}) and $j\textsuperscript{th}$ word (the \textit{modifier}).
\cref{fig:example_dependency_tree} shows examples of dependency trees produced by this model.
We use a probabilistic model where the output $Y$ can more broadly represent a probability distribution over trees, represented by the matrix of arc marginals induced by this distribution (illustrated in \cref{appendix:additional_viz}.)


\begin{figure*}[t]
\centering\small
%\begin{minipage}{.49\textwidth}
\begin{subfigure}[b]{.49\textwidth}
\caption{Baseline (biaffine attention)}
\begin{dependency}[hide label,edge unit distance=1.1ex]
\begin{deptext}[column sep=0.02cm]
Abre \&
a \&
perspectiva \&
de \&
aplicações \&
por \&
prazo \&
mais \&
longos \&
. \\
\end{deptext}
\depedge{1}{3}{1.0}
\depedge[edge unit distance=.8ex]{1}{10}{1.0}
\depedge{3}{2}{1.0}
\depedge{3}{5}{1.0}
\depedge{5}{4}{1.0}
\depedge{5}{7}{1.0}
\depedge[color=purple,thick]{5}{9}{1.0}
\depedge{7}{6}{1.0}
\depedge{9}{8}{1.0}
\deproot[edge unit distance=2.5ex]{1}{}
\end{dependency}
% 'Abre' -> 'perspectiva'
% 'Abre' -> '.'
% 'perspectiva' -> 'a'
% 'perspectiva' -> 'aplicações'
% 'aplicações' -> 'de'
% 'aplicações' -> 'prazo'
% 'aplicações' -> 'longos'
% 'prazo' -> 'por'
% 'longos' -> 'mais'
% 'Abre' -> 'Abre'
\end{subfigure}\quad
%
%
%\begin{minipage}{.49\textwidth}
\begin{subfigure}[b]{.49\textwidth}
\caption{UNN, k=2 (and gold tree)}
\begin{dependency}[hide label,edge unit distance=1.1ex]
\begin{deptext}[column sep=0.02cm]
Abre \&
a \&
perspectiva \&
de \&
aplicações \&
por \&
prazo \&
mais \&
longos \&
. \\
\end{deptext}
\depedge{1}{3}{1.0}
\depedge[edge unit distance=.8ex]{1}{10}{1.0}
\depedge{3}{2}{1.0}
\depedge{3}{5}{1.0}
\depedge{5}{4}{1.0}
\depedge{5}{7}{1.0}
\depedge{7}{6}{1.0}
\depedge[color=purple,thick]{7}{9}{1.0}
\depedge{9}{8}{1.0}
\deproot[edge unit distance=2.5ex]{1}{}
\end{dependency}
% 'Abre' -> 'perspectiva'
% 'Abre' -> '.'
% 'perspectiva' -> 'a'
% 'perspectiva' -> 'aplicações'
% 'aplicações' -> 'de'
% 'aplicações' -> 'prazo'
% 'prazo' -> 'por'
% 'prazo' -> 'longos'
% 'longos' -> 'mais'
% 'Abre' -> 'Abre'
\end{subfigure}
    \caption{Examples of dependency trees produced by the parsing model for a sentence in Portuguese. The baseline model (a)
    erroneously assigns the noun \textit{aplicações} as the syntactic head of the adjective \textit{longos}. The UNN with $k=2$ iterations (b) matches the gold parse tree for this sentence, eventually benefiting from the structural information propagated back from the node $\var{Y}$ after the first iteration.}
    \label{fig:example_dependency_tree}
\end{figure*}

\paragraph{Biaffine parsing.}
A successful model for dependency parsing is the biaffine one
\citep{dozat2016deep, kiperwasser-goldberg-2016-simple}.
This model first computes head representations $H \in \reals^{d \times n}$ and modifier representations $M \in \reals^{d \times n}$,
via a neural network that takes $X$ as input -- here, $d$ denotes the hidden dimension of these representations.
Then, it computes a score matrix as $Z = H^\top V M \in \reals^{n \times n}$, where $V \in \reals^{d \times d}$ is a parameter matrix. 
Entries of $Z$  can be interpreted as scores for each candidate arc.
From $Z$, the 
best tree is found by the Chu-Liu-Edmonds  maximum spanning arborescence algorithm \citep{Chu1965, Edmonds1967}, and
probabilities and marginals by the matrix-tree theorem \citep{koo2007structured,smith2007probabilistic,mcdonald2007complexity,Kirchhoff1847}.

\paragraph{UNN for parsing.}
We now construct an UNN with the same building blocks as this biaffine  model, leading to the factor graph in \cref{fig:factors_all_models}(d).
The variable nodes are $\{\var{X}, \var{H}, \var{M}, \var{Y}\}$,
and the factors are $\{\var{XH}, \var{XM}, \var{HMY}\}$.
Given parameter weight matrices $V, W_\var{H}, W_\var{M} \in \reals^{d \times
d}$ and biases $b_\var{H}, b_\var{M} \in \reals^{d}$,
% \andre{missing some parameters here, I think it should be $W_H$, $W_M$, $b_H$, $b_M$, $V$}
we use multilinear factor energies as follows: 
%\vlad{is the term ``local'' energies defined? do these differ from other
%energies used in the paper?}
%In the case for parsing, we have the following variables and parameters (where $n$ is the sequence length, $d$ is the input dimension (embedding size) and $r$ is the hidden dimension of the network):
% \andre{state the dimensions to be clear}:
%\begin{itemize}
%    \item $X$ - the input sentence $X \in \reals^{d \times n}$.
%    \item $H \in \reals^{r \times n}$ - The heads representations, depends on $X$.
%    \item $M \in \reals^{r \times n}$ - The modifiers representations, depends on $X$.
%    \item $Y \in \reals^{n \times n}$ - The output tree representation (rows are heads, columns are modifiers).
    % \andre{rows are heads, columns are modifiers}
%    \item $V,W \in \reals^{r \times r}$ - Parameters
%\end{itemize}
% \andre{move this part earlier where you define these matrices. we don't need to define $A$ and $B$ explicitly if we use the trace notation above}
%We define the energies for the following factors:
% \andre{I'm appending the matrix form of these equations using trace notation. Trace is the sum of the elements of the diagonal of a matrix. Note that $\mathrm{Tr}(A^\top B) = \mathrm{Tr}(B A^\top) = \mathrm{vec}(A)^\top \mathrm{vec}(B)$}
% \vlad{I have added a macro for DP notation and explained it in the intro. Usage example: $\DP{A}{B}.$}
% \andre{I added negative signs}
%We define bilinear energies between the input and the head and modifier representations:
% \vlad{this is not a sentence, no verb}
\begin{equation}
\begin{aligned}\label{eq:factor_energies_parsing}
    % E_{\var{XH}}(X,H) &= -\sum_{i}h_i^{\top}W_\var{H} x_i = -\DP{H}{W_\var{H} X}\,,\\
    % E_{\var{XM}}(X,M) &= -\sum_{i} m_i^{\top}W_\var{M} x_i = -\DP{M}{W_\var{M} X}\,, \\
    % E_\var{YHM}(Y,H,M) &= -\sum_{ij} y_{ij}(h_i^{\top} V m_j) = -\DP{Y}{H^\top VM}\,.
    E_{\var{XH}}(X,H) &= -\DP{H}{W_\var{H} X}\,,\\
    E_{\var{XM}}(X,M) &= -\DP{M}{W_\var{M} X}\,, \\
    E_\var{YHM}(Y,H,M) &=  -\DP{Y}{H^\top VM}\,.
\end{aligned}
\end{equation}

% \vlad{in code, you also have bias terms, but they're not in the equations} \andre{the bias terms should not be in the factor energies, but in the unary energies, right? check my comment below}
% \tsvm{checked the code and what I think is the case here is that the biases $b_H$ and $b_M$ are there, but we consider them as part of the unary energies. I.e. the linear layers in the code $h_{mlp}$ and $m_{mlp}$ have biases, but they are the ones that correspond to the biases from the unary energies in the equations. Fixed the equations for $E_H(H)$ and $E_M(M)$ according to Andre's suggestion. However $E_Y(Y)$ doesn't have bias - in the equations here and the code and I guess there might be something not OK with it + the entropy term. Let's check these on the meeting together.} -> we checked, it's fine as it is.

%The trilinear energy between the heads, modifiers and the output is:
% \vlad{this is not a sentence, no verb}

%\begin{align}\label{eq:derive_EHMY}
%    E_\var{YHM}(Y,H,M) &= -\sum_{ij} y_{ij}(h_i^{\top} V m_j) \nonumber \\
    % &= -\mathrm{Tr}(Y^\top H^\top V M)
%    &= -\DP{Y}{H^\top VM}\,.
    % \andre{= \mathrm{Tr}(Y^\top H^\top V M)}
%\end{align}

% \andre{I don't find the inner product bracket notation particularly useful... perhaps we can just use trace everywhere? it makes it closer to the notation we used for vectors earlier when using bilinear factor energies} \vlad{We can pick one or the other, but I agree no need to use both. I do think I prefer bracket, but not strongly.}\tsvm{we decided on brackets everywhere, I need to fix it.}
% \andre{we may want to point out that the energy above is trilinear}
%\begin{equation}
%    E_H(h_i) = \frac{1}{2}||h||^2 + \iota_{\geq 0}(h_i)
%\end{equation} 
For $\var{H}$ and $\var{M}$, we use the ReLU regularizer,
\begin{equation}\label{eq:unary_energies_parsing}
\begin{aligned}
    E_\var{H}(H)
    % &= -\mathrm{Tr}(1_n b_H^\top H) +
    &= -\DP{b_\var{H} \otimes 1_n}{H} +
    \frac{1}{2}\|H\|^2 + \iota_{\geq 0}(H)\,\\
    E_\var{M}(M)
    % &= -\mathrm{Tr}(1_n b_M^\top M) +
    &= -\DP{b_\var{M} \otimes 1_n}{M} +
    \frac{1}{2}\|M\|^2 + \iota_{\geq 0}(M)\,.\\
\end{aligned}
\end{equation}
For $\var{Y}$, however, we employ a structured entropy regularizer:
\begin{equation}
\begin{aligned}
    E_\var{Y}(Y) &= -\entropy_\mathcal{M}(Y) + \iota_{\mathcal{M}}(Y)\,,
\end{aligned}
\end{equation}
where $\mathcal{M}=\conv(\mathcal{Y})$ is the marginal polytope
\citep{wainwright2008graphical,martins2009polyhedral},
the convex hull of the adjacency matrices of all valid non-projective dependency trees (\cref{fig:example_marginals}), and $\entropy_\mathcal{M}(Y)$ is the maximal entropy over all distribution over trees with arc marginals $Y$:
%containing the arc marginals that are realizable for an arc-factored model 
\begin{equation}
\entropy_\mathcal{M}(Y) \coloneqq \max_{\alpha \in \triangle_{|\mathcal{Y}|}}
\mathcal{H}(\alpha) 
~\text{s.t.}~
\mathbb{E}_{A\sim\alpha}[A] = Y
\,.
\end{equation}
% \andre{I think we are missing the bias terms here (linear functions). It should be $-\mathrm{Tr}(1_n b_H^\top H) + \frac{1}{2}\|H\|^2 + \iota_{\geq 0}(H)$ and $-\mathrm{Tr}(1_n b_M^\top M) + \frac{1}{2}\|M\|^2 + \iota_{\geq 0}(M)$} 
% \andre{do we use a bias term for $E_Y(Y)$ as well?}\tsvm{No. See my comment above and let's discuss at the meeting.}
%\begin{equation}
%    E_\var{Y}(Y) = -\entropy(Y) + \iota_{\mathcal{M}}(Y),
%\end{equation}
%where 
%$\entropy$ is the entropy of the tree distribution with arc marginals $Y$ (computable through the matrix tree theorem), and $\mathcal{M}$ is the marginal polytope, containing the arc marginals that are realizable for an arc-factored model \citep{wainwright2008graphical,martins2009polyhedral}.
%Here, we do not have a bias term for the energy $E_\var{Y}(Y)$, because the dimension of the output $Y \in \reals^{n \times n}$ depends on the (variable) sequence length. 
%and having a bias term would mean preference for specific positions, which does not make sense in the current context.
% \vlad{not sure what this notation is}
% \andre{At some point, we need to say that we're using $Y$ not just as a binary matrix indicating a tree but also as a convex combination of trees, i.e., a matrix of arc marginals.} \vlad{example or small figure maybe}
% \andre{there is a clash of notation btw entropy $H(Y)$ and matrix $H$, we should prob pick a different notation for the entropy}

%\begin{equation}\label{eq:derive_H_1}
%\begin{split}
%    H = \argmin_{H}(E_{XH}(X,H)  \\
%    + E_{HMY}(H.M,Y) \\
%    + E_H(H))
%\end{split}
%\end{equation}

% We will present the energies in vector form, where we present $vec(M)$ as the vectorized form of matrix $M$, i.e. the columns of the matrix stacked on top of each other in a vector. \andre{we don't need to have this part here, if we use the trace vector notation I added above (btw I think there are some mistakes below with transposes).}

% \begin{equation}\label{eq:derive_EXH}
% \begin{split}
%     E_{XH}(X,H) = \sum_{i}h_i^{T}W_Hx_i = \DP{H}{W_H X}
%     % \sum_{i}a_i^{T}x_i = vec(A)vec(H), \\
%     % \text{where} \quad a_i = W_Hx_i \quad
%     % \text{and} \quad A=W^{T}H \andre{A=W_H X}
% \end{split}
% \end{equation}

% \begin{equation}\label{eq:derive_EHMY}
% \begin{split}
%     E_{YHM}(Y,H,M) = \sum_{ij} y_{ij}(h_i^{T} V m_j) = \\
%     \sum_ih_i^T(\sum_jy_{ij}Vm_j) = \\
%     % \DP{B}{H}
%     % vec(B^T)vec(H),\\
%     % \text{where} \quad B=VMY
%     \DP{H}{V\DP{Y}{M}}
% \end{split}
% \end{equation}


\paragraph{Derivation of block coordinate descent updates.}
% \andre{start a new subsection here where you derive the block coordinate descent updates for each of the variables. then, point out the similarity of each update and the bilinear model of \url{https://arxiv.org/pdf/1611.01734.pdf}; we also need to cite Kipperwasser \& Goldberg}

To minimize the total energy,
we iterate between updating $H$, $M$ and $Y$ $k$ times, similar to the unstructured case. %We use coordinate descent and calculate each variable as a minimization of the sum of the energies of the factors in which it appears.
%We now derive the coordinate descent updates for each variable.
%These coordinate descent updates are similar to the computation performed in the biaffine attention model. 

The updates for the heads and modifiers work out to: 
\begin{equation}
\begin{aligned}
\label{eq:derive_HM}
\nextit{H} &= \relu(W_\var{H} X +  b_\var{H} \otimes 1_n + V\currit{M}\currit{Y}^\top)\,,\\
\nextit{M} &= \relu(W_\var{M}X + b_\var{M} \otimes 1_n + V^\top {H}\currit{Y})\,.
\end{aligned}
\end{equation}
%
%\begin{equation}\label{eq:derive_H}
%\begin{split}
%H = \argmin_H( \DP{H}{W_H X}\\
%+ \DP{Y}{H^\top V M} \\
%+ \psi(H) ) \\
%= \relu(A+B) \\
%= relu(W_HX + VMY^T)
%\end{split}
%\end{equation}
%%% 
%%% \begin{equation}
%%% \begin{aligned}
%%% \label{eq:derive_H}
%%% \nextit{H} &= \argmin_H E(X, H, \currit{M}, \currit{Y}) \\
%%% %&= \argmin_H E_\var{XH}(X,H)\!+\!E_\var{HMY}(H,\currit{M}\!,\currit{Y})\!+\!E_\var{H}(H)\\
%%% % &= \argmin_{H \ge 0} -\mathrm{Tr}(H^\top (W_H X + b_H 1_n^\top + VMY^\top) \nonumber\\
%%% &= \argmin_{H \ge 0} -\DP{H}{W_\var{H} X + b_\var{H} 1_n^\top + VMY^\top}\\
%%% &= \relu(W_\var{H} X b_\var{H} 1_n^\top + V\currit{M}\currit{Y}^\top)\,.
%%% \end{aligned}
%%% \end{equation}
%%% % \andre{we're dropping the iteration number from the first to the subsequent lines}
%%% 
%%% % \begin{equation}\label{eq:derive_H}
%%% % \begin{split}
%%% % H = \argmin_H vec(A)^Tvec(H)\\
%%% % + vec(B)^Tvec(H) \\
%%% % + \psi(H) \\
%%% % = \relu(A+B) \\
%%% % = relu(W_HX + VMY^T)
%%% % \end{split}
%%% % \end{equation}
%%% 
%%% Similar to \cref{eq:derive_H}, the update for $\var{M}$ is
%%% \begin{equation}\label{eq:derive_M}
%%% \nextit{M} = \relu(W_\var{M}X + b_\var{M} 1_n^\top + V^\top \nextit{H}\currit{Y})
%%% \end{equation}
%%% 
For $\var{Y}$, however, we must solve the problem
%Finally, the output assignment of $\var{Y}$ is
\begin{equation}
\begin{aligned}\label{eq:derive_Y}
    \nextit{Y} 
    %&= \argmin_Y E_\var{HMY}(H,M,Y) + E_\var{Y}(Y)\\
    % &= \argmin_{Y \in \mathcal{M}} -\mathrm{Tr}(Y^\top H^\top VM)\nonumber\\
    &= \argmin_{Y \in \mathcal{M}} -\DP{Y}{{H}^\top V{M}}
-\entropy_\mathcal{M}(Y)\,.\\
    %&= \mathrm{marginals}(\nextit{H}^\top V\nextit{M}).
\end{aligned}
\end{equation}
% \vlad{in the middle line the entropy term got lost}
This combinatorial optimization problem corresponds to \emph{marginal 
inference} \citep{wainwright2008graphical}, 
a well-studied computational problem in structured prediction that appears in all probabilistic models. 
While generally intractable, for non-projective dependency
parsing it may be computed in time $\mathcal{O}(n^3)$ via
%first computing the score matrix $Z = H^\top VM$ and then using
the aforementioned matrix-tree theorem, the same algorithm required to compute the structured likelihood loss.% 
\footnote{During training, the matrix-tree theorem can be invoked only once to compute both the update to $Y$ as well as the gradient of the loss, since 
$\nabla \log p(\var{Y}=Y_\text{true}) = 
Y_\text{true}
- \hat{Y}$.}
%-- the same procedure used to compute the
%likelihood loss in probabilistic biaffine parsers \citep{dozat2016deep, kiperwasser-goldberg-2016-simple}.
%\vlad{I'm pretty sure Kiperwasser and Goldberg never compute the likelihood loss
%but instead they use a marign loss. How about dozat?}

% \andre{Provide some intuition for these updates. Say that,
With zero initialization, the first iteration yields the same hidden representations
and output as the biaffine model, assuming the updates are performed
in the order described.
%order of updating the variables is $H \rightarrow M \rightarrow Y$ or $M \rightarrow H \rightarrow Y$.
% \vlad{assuming update order HMY or MHY right? The "unrolling lemma" Andre suggested seems narratively useful here.}
The extra terms involving $VMY^\top$ and $V^\top H Y$ enable the current prediction for $Y$ to influence neighboring words, which leads to a more expressive model overall.
%might lead to a more consistent tree with multiple iterations. %This is why the UNN can be useful for structured prediction problems.
%\vlad{This last few sentences here need attention}

%\paragraph{Initialization}
%With coordinate descent, each variable is updated individually from the values of the other variables it depends on, according to the equations above. This means that we need to initialize the hidden and output variables. Unlike the unstructured case, here it is not trivial to come up with different methods for initialization, so we are initializing the necessary variables with zeroes.
%\vlad{do we want this paragraph here? maybe we make a bigger discussion about
%initialization in general, using Tsveti's result from the completion experiment}

% \begin{figure*}[ht!]
%     \centering
%     \includegraphics[width=12cm]{img/factor_graph_structured_unn}
%     \caption{Factor graph representing an example for structured UNN for dependency parsing.}
%     \label{fig:factor_graph_structured_unn}
% \end{figure*}

\begin{table}[t]
    \caption{Structured UNN parsing results.
    Columns show the number of UNN iterations.
    %The three table sections show UAS, MA, SA metrics for each language.
    The best result per row is rendered in bold.
    }
    \vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
    \begin{tabular}{*6c}
    \toprule
    % Language & \multicolumn{5}{c}{$k$} \\
    % \midrule
    Language & $k=1$ & $k=2$ & $k=3$ & $k=4$ & $k=5$ \\
    \midrule 
    \multicolumn{6}{c}{Unlabeled attachment score} \\
    \midrule
    % UAS & & & & \\
    AF & \textbf{89.09} & 88.98 & 88.40 & 87.77 & 88.46 \\
    AR & \textbf{85.62} & 84.94 & 84.22 & 83.69 & 83.63 \\
    CS & 93.79 & \textbf{93.83} & 93.82 & 93.60 & 93.77 \\
    EN & 91.96 & 91.86 & 91.09 & \textbf{91.99} & 91.51 \\
    FA & \textbf{83.41} & 83.27 & 82.95 & 83.37 & 83.27 \\
    HU & 85.11 & \textbf{85.77} & 84.47 & 85.13 & 84.09 \\
    IT & \textbf{94.76} & 94.43 & 94.35 & 94.59 & 94.45 \\
    PT & 96.99 & 97.00 & 96.83 & \textbf{97.06} & 96.90 \\
    SW & \textbf{91.42} & 90.92 & 91.30 & 91.08 & 90.98 \\
    TE & 89.72 & 89.72 & \textbf{90.00} & 88.45 & 87.75 \\

    \midrule
    \multicolumn{6}{c}{Modifier list accuracy} \\
    \midrule
    AF &  \textbf{74.10} & 72.60 & 72.90 & 71.78 & 72.01 \\
    AR &  \textbf{70.44} & 69.29 & 68.41 & 68.08 & 68.19 \\
    CS &  84.46 & 84.82 & \textbf{84.93} & 84.12 & 84.49 \\
    EN &  79.08 & 77.73 & 75.20 & 78.90 & \textbf{79.44} \\
    FA &  64.80 & \textbf{66.75} & 65.28 & 66.67 & 65.85 \\
    HU &  64.13 & \textbf{66.07} & 64.37 & 62.91 & 64.13 \\
    IT &  \textbf{85.32} & 83.59 & 83.71 & 83.94 & 84.05 \\
    PT &  90.10 & \textbf{90.69} & 90.39 & 90.66 & 90.49 \\
    SW &  \textbf{79.07} & 78.37 & 78.52 & 78.60 & 78.24 \\
    TE &  72.87 & 72.87 & \textbf{73.68} & 66.80 & 65.99 \\

    \midrule
    \multicolumn{6}{c}{Exact match} \\
    \midrule
    AF &  \textbf{37.70} & 33.88 & 34.43 & 33.88 & 32.79 \\ 
    AR &  19.44 & 19.29 & 18.36 & \textbf{19.91} & 18.36 \\
    CS &  59.17 & 60.76 & \textbf{60.92} & 59.42 & 59.84 \\
    EN &  \textbf{48.59} & 44.37 & 40.14 & 43.66 & 44.37 \\
    FA &  21.52 & 22.15 & 22.78 & \textbf{24.68} & 23.42 \\
    HU &  21.13 & 23.40 & \textbf{24.15} & 23.40 & 21.51 \\
    IT &  \textbf{64.93} & 63.54 & 62.85 & 63.89 & 64.24 \\
    PT &  73.24 & \textbf{74.86} & 73.89 & 74.43 & 74.11 \\
    SW &  \textbf{54.62} & 52.38 & 54.13 & 53.94 & 52.67 \\
    TE &  75.69 & 77.08 & \textbf{79.17} & 71.53 & 70.14 \\
    \bottomrule
    \end{tabular}
    \end{sc}
    \end{small}
    \end{center}
    \label{table:parsing_results}
\end{table}



\paragraph{Experiments.}

%We experiment with the UNN for parsing described above. 
We test the architecture on several datasets from Universal Dependencies 2.7 \citep{universal-dependencies-2.7}, covering different language families and dataset size: Afrikaans (AfriBooms), Arabic (PADT), Czech (PDT), English (Partut), Hungarian (Szeged), Italian (ISDT), Persian (Seraji), Portuguese (Bosque), Swedish (Talbanken), and Telugu (MTG). Performance is measured by three metrics:
\begin{itemize}
    \item Unlabeled attachment score (UAS): a fine-grained, arc-level accuracy metric.
    \item Modifier list accuracy: the percentage of head words for which \textit{all} modifiers were correctly predicted. For example, in \cref{fig:example_dependency_tree}, the baseline correctly predicts all modifiers for the words \emph{perspectiva, abre, longos}, but not for the words \emph{aplicações, prazo}.
    \item \looseness=-1
    Exact match: the percentage of sentences for which the entire parse tree is correct; the harshest of the metrics.
\end{itemize}
The latter, coarser measures can give more information whether the model is able to learn global relations, not just how to make local predictions correctly (\textit{i.e.}, when only prediction of the arcs is evaluated).

Our architecture is as follows: First, we pass the sentence through a BERT model (\textsc{bert-base-multilingual-cased}, fine-tuned during training, as directed networks can be added as components to UNNs, as mentioned in \cref{section:unn}) 
and get the word representations of the last layer. These representations are
the input $x$ in the UNN model. Then, we apply the parsing model described in
this section. The baseline ($k=1$) corresponds to a biaffine parser using BERT features.
%is a BERT model (we use
%\textsc{bert-base-multilingual-cased}) with a parser on top, which is equal to a
%UNN with a single iteration and zero initialization of the output $y$. We fine-tune the BERT weights. 
The learning rate for each language is chosen via grid search for highest UAS on the validation set for the baseline model. We searched over the values $\{0.1, 0.5, 1, 5, 10\} \times 10^{-5}$.
% \vlad{do you mean grid search? fine-tuning here usually means updating the weights of a pretrained model, a meaning htat you've already used in the previous sentence} 
In the experiments, we use $10^{-5}$ for Italian and $5 \times 10^{-5}$ for the other languages. 
We employ dropout regularization, using the same dropout mask for each variable throughout the inner coordinate descent iterations, so that dropped values do not leak.


The results from the parsing experiments are displayed in \cref{table:parsing_results}.
The numbers in the table show results on the test set for the highest validation accuracy epoch.
We see that some of the languages seem to benefit from the iterative procedure of UNNs (CS, HU, TE), while others do not (EN, AF), and little difference is observed in the remaining languages. 
In general, the baseline ($k=1$) seems to attain higher accuracies in UAS (individual arcs), but most of the languages have overall more accurate structures (as measured by modifier list accuracy and by exact match)
for $k>1$. 
\cref{fig:example_dependency_tree} illustrates with one example in Portuguese. 

%slight improvements for multiple iterations for most languages, but the best number of iterations is not consistent throughout the languages. \andre{the last sentence doesn't sound very convincing. could we say that, for UAS, the baseline $k=1$ seems a good strategy, but for evaluating full structures, $k \in \{2,3\}$ seem generally more effective (explain why) and too many iterations (e.g. $k=5$) seem harmful} \andre{actually it looks like $k=1$ is better than anything else on everything -- wins 5 times for UAS, 4 times in mod acc, 4 times on exact match}



==> [ICML 2022] Undirected Neural Networks/introduction.tex <==
% \andre{We could start with a motivating sentence here about how neural networks and graphical models for structured prediction are two different toolboxes, and how we put them together. E.g. ``Factor graphs have historically been a very appealing toolbox for representing structured prediction problems in NLP, with wide applications to parsing, dialogue, and relation extraction (cite a few papers). In the last years, neural networks have taken over as the model of choice for tackling these applications. Unlike factor graphs -- which capture and emphasize the modularity of the problem -- neural architectures tend to be monolithic, relying on rich representations captured at the encoder level (often pre-trained), which are then propagated to a task-specific decoder. In this paper, we combine the representational strengths of factor graphs and neural networks by proposing \textbf{undirected energy-based models}.''}

% \vlad{\begin{itemize}
%     \item fix notation issues
% \end{itemize}}
\looseness=-1
Factor graphs have historically been a very appealing toolbox for representing structured prediction problems \citep{bakir2007predicting,smith2011linguistic,nowozin2014advanced}, with wide applications to vision and natural language processing applications.  
% \tsvm{cite a few papers} \andre{make this a bit broader and not just about NLP applications?}. 
In recent years, neural networks have taken over as the model of choice for tackling many such applications. Unlike factor graphs\,--\,which emphasize the modularity of the problem\,--\,neural networks typically work end-to-end, relying on rich representations captured at the encoder level (often pre-trained), which are then propagated to a task-specific decoder. 

In this paper, we combine the representational strengths of factor graphs and neural networks by proposing \textbf{undirected neural networks} (UNNs) -- a framework in which outputs are not computed by evaluating a composition of functions in a given order, but are rather obtained \textit{implicitly} by minimizing an energy function which factors over a graph. 
For particular choices of factor potentials, UNNs subsume many existing architectures, including feedforward, recurrent, and self-attention neural networks, auto-encoders, and networks with implicit layers. 
When coupled with a coordinate descent algorithm to minimize the energy, the computation performed by an UNN is similar (but not equivalent) to a neural network sharing parameters across multiple identical layers. 
Since UNNs have no prescribed computation order, the exact same network can be used to predict any group of variables (outputs) given another group of variables (inputs), or vice-versa (\textit{i.e.}, inputs from outputs) enabling new kinds of joint models. 
%
% the undirected neural networks present a different point of view on the \andre{this sentence is incomplete}
%
% The goal we want to achieve is to train different modules for specific subtasks for a bigger task and train those modules separately, as well as together for the downstream task. In this section, we propose Undirected Neural Networks (UNN) - an energy-based model which allows training of several modules together.
%
% In this paper, we define the concept of UNN and we validate it with some preliminary experiments on several toy tasks. We explain the concept, the preliminary experiments, and proposed extensions.
%
% The goal of the energy-based model is to optimize the model energy. The \emph{energy} can be described as a score of the model (a measure of compatibility of the variables). \citep{lecun2006tutorial}.
% The inference, i.e. making a prediction or decision, consists in setting the value of observed variables and finding values of the remaining variables that minimize the energy. To describe the model of UNNs, we will go through some known energy-based models - Boltzmann Machines.
%
In sum, our contributions are:

\begin{itemize}
    \item We present UNNs and show how they extend many existing neural architectures.   
    % based on energy updates  by looking at the model as an undirected factor graph \andre{it's not just a ``view'' right? Our model is more general than standard neural networks, the way this is written seems to suggest we're just reinterpreting something that already exists}.
    %for particular choices of factor potentials, they subsume most existing architectures, including feedforward, recurrent, and self-attention neural networks, auto-encoders, and networks with implicit layers.
    % \andre{we can say here that our networks (maybe call them Undirected Energy-Based Models), for particular choices of factor potentials, subsume most existing architectures, including feedforward, recurrent, and self-attention neural networks, auto-encoders, and networks with implicit layers (I need to remember how to the latter was done)}
    \item We provide a coordinate descent inference algorithm, which, by an
    ``unrolling lemma'' (\cref{lemma:unrolling}),
    can reuse current building blocks from feed-forward networks in a modular way.
    % \andre{maybe rephrase this as ``we provide a coordinate-descent energy minimization algorithm to perform computation in this factor graph which allows reusing current building blocks in a modular way and is guaranteed to always decrease the energy.''}
%\item This results on a compact, modular factor graph for performing structured prediction tasks, which we illustrate with natural language parsing.
    % \item We compare this model to other models that can model structures (SPEN)... \andre{this is an interesting point. I believe reviewers would like to see this comparison e.g. for parsing, but it may take some time to implement the SPEN baseline. In any case I think we should draw the parallel between the two models at least in the theoretical sections since both are energy based models}
    % \item We explore undirected neural networks with different architecture for structured and unstructured tasks - classification, generation, parsing, multitask classification. We also demonstrate a basic implementation of undirected attention and evaluate it on sequence completion. \andre{We develop and experiment with multiple factor graph architectures, tackling both structured and unstructured tasks, such as ... We develop a new kind of ``undirected'' attention mechanism and demonstrate its usefulness on a simple sequence completion task.}
    \item We develop and experiment with multiple factor graph architectures, tackling both structured and unstructured tasks, such as natural language parsing, image classification, and image prototype generation. We develop a new undirected attention mechanism and demonstrate its suitability for sequence completion.\footnote{The source code is on \href{https://github.com/deep-spin/unn}{https://github.com/deep-spin/unn}.}
    % \andre{and depedency parsing, which covers both unstructured and structured tasks}.
\end{itemize}

%In the remaining part of the paper, we describe the model as follows: in Section~\ref{section:unn} we describe our model - definition of the factor graph, selection of the factors energies, energy minimization with coordinate descent, relation to existing architectures. Section~\ref{section:related_work} describes existing architectures that can be derived as a special cae of UNNs as well as other existing architectures with an idea close to UNNs. In sections \ref{section:experiments_parsing}, \ref{section:experiments_attention}, \ref{section:experiments_mnist}, we demonstrate the flexibility of the undirected neural networks with several applications.

% hopeful other contributions:

% \begin{itemize}
%     \item Advantages/disadvantages wrt to SPENs for the structured factors case (easier inference and training?)
%     \item Relation with implicit layers (do UNN subsume them?)
%     \item UNNs very general and subsume other frameworks (incl. FFNNs and SPENs)
%     \item generate x given y (eg for mnist)
%     \\ \quad (rel to Grathwohl EBM)
%     \\ \quad (pitch as prototype rather than sampler)
%     \\ \quad (make stochastic?)
% \end{itemize}

\paragraph{Notation.}
We denote vector values as $a$, matrix and tensor values as $A$, and abstract factor graph variables as $\var{A}$.
The Frobenius inner product of two tensors with matching dimensions $A, B \in \reals^{d_1 \times \ldots \times d_n}$ is
$\DP{A}{B} \coloneqq \sum_{i_1=1}^{d_1} \ldots \sum_{i_n=1}^{d_n} a_{i_1\ldots{}i_n} b_{i_1 \ldots i_n}$. For vectors
$\DP{a}{b}=a^\top b$ and for matrices $\DP{A}{B}=\Tr(A^\top B)$.
The Frobenius norm is $\|A\| \coloneqq \sqrt{\DP{A}{A}}$.
Given two tensors $A \in \reals^{c_1, \ldots, c_m}, B \in \reals^{d_1, \ldots, d_n}$, their outer product is
$(A \otimes B)_{i_1, \ldots, i_m, j_1, \ldots, j_n} = a_{i_1, \ldots, i_m} b_{j_1, \ldots, j_m}$. For vectors, $a \otimes b = ab^\top$.
%The inner product of two vectors $a,b \in \reals^n$ is denoted as $\DP{a}{b} \coloneqq \sum_{i=1}^n a_ib_i$,
%and the Euclidean norm as $\|a\| = \sqrt{\DP{a}{a}}$.
%We denote the inner product of matrices
%$A, B \in \reals^{m \times n}$ as
%$\DP{A}{B} \coloneqq \sum_{i=1}^m \sum_{j=1}^n a_{ij} b_{ij}$, and the Frobenius matrix norm as $\|A\| = \sqrt{\DP{A}{A}}$.
%If $\vecz(A)$ is the flattening reshape operator from $\reals^{m \times n}$ to $\reals^{mn}$, then $\DP{A}{B} = \vecz(A)^\top\vecz(B) = \mathrm{trace}(A^\top B)$.
We denote the $d$-dimensional vector of ones as $1_d$ (or tensor, if $d$ is a tuple.)
The Fenchel conjugate of a function $\Psi : \reals^d \rightarrow \reals$ is
$\Psi^*(t) \coloneqq \sup_{x \in \reals^d} \DP{x}{t} - \Psi(x)$. When $\Psi$ is strictly convex,
$\Psi^*$ is differentiable, and
$(\nabla\Psi^*)(t)$ is the unique maximizer
$\argmax_{x \in \reals^d} \DP{x}{t} - \Psi(x)$. 
%The optimal value of an optimization variable is denoted
%The star notation is not to be confused with the optimality notation 
%$x_\star$.
%which denotes the optimal value of a variable.
% If $\Tr(Z) = \sum_i z_{ii} $ is the matrix trace of a square matrix $Z$, then $\DP{A}{B} = \Tr(A^\top B) = \Tr(B^\top A)$.
% \item We define the \textbf{constraints on the variables} with $\iota$. For example, $\iota_{\{0,1\}^{N}}(x)$ means constraint on $x$, i.e. $x$ needs to be $N$ zeros or ones. 
We denote the non-negative reals as
$\reals^d_+ \coloneqq \{ x \in \reals^d : x \geq 0 \}$,
and the $(d-1)$-dimensional simplex as
$\triangle_d \coloneqq \{ \alpha \in \reals^{d}_+, \DP{1_d}{\alpha}=1\}.$
The Shannon entropy of a discrete distribution $y \in \triangle_d$ is
$\entropy(y) \coloneqq -\sum_i y_i \log y_i$.
The indicator function %of a set $\mathcal{X}$ is denoted and defined as 
$\iota_{\mathcal{X}}$ is defined as
$\iota_{\mathcal{X}}(x) \coloneqq 0$ if $x \in \mathcal{X}$, and $\iota_{\mathcal{X}}(x) \coloneqq +\infty$ otherwise.

%Given a set $S=\{s_1, \ldots, s_d\}$,
%the Shannon entropy of a structured marginal distribution over its convex hull is
%$\entropy(y) : \conv(S) \to \reals_+$, 
%$\entropy(y) \coloneqq \max \{\sum_i -\alpha_i \log \alpha_i : \alpha \in \triangle_{|S|}, \sum_{i=1}^k \alpha_i s_i = y\}$ \andre{this definition is not very standard and it may appear confusing. Maybe we can just define the standard entropy here and refer to the general one inline in the parsing section? We should also connect $\conv(S)$ to the marginal polytope (OTOH the definition is quite elegant)}.


==> [ICML 2022] Undirected Neural Networks/related_work.tex <==
\section{Related Work}\label{section:related_work}

% \andre{move this section to the end before the conclusions?}

% \andre{this section needs some work. most of it feels a bit redundant to what we present (and well) in sec 2. I suggest we just write 1-2 sentences (not individual paragraphs) reminding that our work subsumes FFNNs, AEs, related to BMs, etc, and keep only the other paragraphs that focus on the connections that have not been made yet. For each related work we disucss we need to be precise and cite the relevant literature, I feel that it some parts we are handwaving a bit.}

 %In \cref{section:unn} we discuss how our model subsumes feed-forward networks, auto-encoders, and implicit layers. In this section, we explain how it relates to other existing architectures. 
Besides the models mentioned in \cref{section:unn}  which may be regarded as particular cases of UNNs, other models and architectures, next described, bear relation to our work. 

% \paragraph{Feed-Forward Networks}
% Per Section~\ref{section:unn},
% UNN with $k=1$ iterations and initialization $\initit{y}=0$, represent a feed-forward neural network with one hidden layer. The same is true for multiple hidden layers, when the updates of the hidden layers follow their order in the network. \andre{we probably don't need this paragraph, this connection has already been pointed out in Sec 2}

\paragraph{Probabilistic modeling of joint distributions}
% The UNNs considered in our paper can be regarded as a particular case \andre{can they? this contradicts the fact pointed out below that our variables are not discreteand that our model is not probabilistic} of sparsely connected Boltzmann machines where unit connections are specified according to a factor graph \andre{this might sound a bit confusing, since our factor graph takes input variables that are vectors, whereas it looks like the sparsely connected BM we're mentioning are sparse wrt individual variables. Also, if our work relates to this, we should cite the relevant literature. Which papers presents/covers sparsely connected Boltzmann machines? perhaps we should not bring BMs again in this related work section, since we're already discussing that after Lemma 1}. Our work departs from this line of research in two ways: (1) our variables are continuous and not discrete, enabling inference with continuous optimization, and (2) the goal of our network is not to compute a probability distribution over the observed variables, but rather to learn a prediction function, which avoids having to approximate intractable partition functions.

Our work draws inspiration from the well-known Boltzmann machines and Hopfield networks \citep{ackley1985learning,smolensky1986information,hopfield1984neurons}. 
We consider deterministic networks whose desired configurations minimize an energy function which decomposes as a factor graph. In contrast, 
many other works have studied probabilistic energy-based models (EBM) defined as Gibbs distributions, as well as efficient methods to learn those distributions and to sample from them \citep{ngiam2011learning,du_mordatch}. 
% which model the joint distribution of $x$ and $y$ using energy-based models, which require Markov chain Monte Carlo (MCMC) and rely on drawing many samples, therefore are slower than our model. 
Similar to how our convolutional UNN can be used for multiple purposes
in \cref{section:experiments_mnist}, 
\citet{Grathwohl2020Your} reinterprets standard discriminative classifiers $p(\var{Y}|\var{X})$ as an EBM of a joint distribution $p(\var{X},\var{Y})$. 
% \vlad{Not sure i agree with the next sentence, EBMs are basically undirected as well. Also it's a bit of a low attack: ``none of these works used the term we invented today''}
% None of these works, however, considers \textit{undirected} networks.
% \vlad{I suggest instead:}
Training stochastic EBMs requires Monte Carlo sampling or auxiliary 
networks \citep{grathwohl2020learning}; in contrast,
our deterministic UNNs, more aligned conceptually with deterministic EBMs \citep{lecun2006tutorial}, eschew probabilistic modeling in favor of
more direct training.
Moreover, our UNN architectures closely parallel feed-forward networks and reuse their building blocks, uniquely bridging the two paradigms.

% \tsvm{mention that more broadly there are probl. models...}
% \vlad{relwork: probabilistic modeling of the joint(x,y) using nn – requires MCMC, much slowerthan ours, many samples.}

% \paragraph{Hopfield Networks}
% % \vlad{does the paper use the word modern? in any case in latex the correct way to write quotes is ``like this''}
% Recent work \citep{ramsauer2020hopfield} shows that the attention mechanism of the widely used transformer model \citep{vaswani2017attention} is equal to the update rule of a Hopfield network with continuous states \citep{hopfield1984neurons}. This work proposes a ``modern Hopfield network'' with continuous states with an update rule which ensures global convergence to stationary points of the energy (local minima or saddle points). \andre{maybe 1 brief sentence explaining how our work differs/relates?}

% \tsvm{move related work at the end. cite universal tranformers...} \andre{universal transformers paper: \citep{dehghani2018universal}}


% \subsection{Implicit Layers}
% With our proposed model, we can represent networks with implicit layers. The implicit layers \citep{duvenaud2020deep}, in contrast with feed-forward layers, do not specify how to compute the output from the input, but rather specify conditions that the output layer should specify.
% In our framework, if we pick $E_{XH}$ to be some more complicated function of $x$ and $h$ (not simply a bilinear + pointwise penalty one) then computing $h^\star$ given $x$ is an "implicit layer" that requires optimization.
% \vlad{I think what Andre means is that if in our framework we pick $E_{XH}$ to be some more complicated function of $x$ and $h$ (not simply a bilinear + pointwise penalty one) then computing $h^\star$ given $x$ is an "implicit layer" that requires optimization. So I think our formalism does "subsume" implicit layers, although none of our concrete experiments use this. We should explain this connection somewhere in text.}


\paragraph{Structured Prediction Energy Networks (SPENs)}
We saw in \cref{section:experiments_parsing} that UNNs can handle structured outputs. An alternative framework for expressive structured prediction is given by SPENs \citep{belanger2016structured}. 
Most SPEN inference strategies require gradient descent, often with higher-order gradients for learning \citep{belanger2017end}, or training separate inference networks \citep{tu-etal-2020-improving}.
UNNs in contrast, are well suited for coordinate descent
inference: a learning-rate free algorithm with 
updates based on existing neural network building blocks.
%(affine and convolutional layers, nonlinear activations).
An undirected variant of SPENs would be similar to the MLP factor graph in \cref{fig:factors_all_models}(b), but with $\var{X}$ and $\var{Y}$ connected to a joint, higher-order factor, rather than via a
chain $\var{X-H-Y}$.
%\vlad{if we have space, maybe draw this factor? I can't quite tell what it's supposed to be.}
% \andre{maybe point out that a undirected variant of SPENs would be similar to the MLP FG in our figure, but with X and Y connected in a factor instead of a chain X-H-Y?}

% \andre{We should talk here about some classic architectures that are undirected, such as Boltzmann machines and Hopfield networks. E.g. ``Our work draws heavy inspiration in classical models such as Boltzmann machines and Hopfield networks. In fact, the undirected energy based models considered in our paper can be regarded as a particular case of sparsely connected Boltzmann machines where unit connections are specified according to a factor graph. Our work departs from this line of research in two ways: (1) our variables are continuous and not discrete, enabling inference with continuous optimization, and (2) the goal of our network is not to compute a probability distribution over the observed variables, but rather to learn a prediction function, which avoids having to approximate intractable partition functions.}

% \andre{A paragraph about SPENs, with advantages and disadvantages. One point to mention here is that current algorithms to make preditions with SPENs involve gradient-descent algorithms and often require higher-order gradients for learning, or complicated architectures with separate networks for inference and for computing the energy. Our models, in contrast, by relying on coordinate-descent energy minimization, can be easily learned with first-order gradients and existing building blocks.}


% \paragraph{Autoencoders}
% We show in the experiments (Section~\ref{section:experiments_mnist} and \ref{section:experiments_attention}) how with our model the input variables can be easily updated. This resembles the update of the autoencoders. \andre{we probably don't need this paragraph, this connection has already been pointed out on other parts of the paper}

\paragraph{Universal transformers and Hopfield networks}
% \andre{maybe merge this paragraph with the Hopfield networks one?}
In \cref{section:experiments_attention} we show how we can implement self-attention with UNNs. Performing multiple energy updates resembles -- but is different from -- transformers \citep{vaswani2017attention} with shared weights between the layers. 
Our perspective of minimizing UNNs with coordinate descent using a fixed schedule and this unrolling is similar (but not exactly the same due to the skip connections) to having deeper neural networks which shared parameters for each layer. Such an architecture is the Universal Transformer \citep{dehghani2018universal}, which applies a recurrent neural network to the transformer encoder and decoder.
% \vlad{The above sentence kind of says this. Maybe just emphasize this again when discussing universal transformer} 
Recent work \citep{ramsauer2020hopfield} shows that the self-attention layers of transformers can be regarded as the update rule of a Hopfield network with continuous states \citep{hopfield1984neurons}. This leads to a ``modern Hopfield network'' with continuous states and an update rule which ensures global convergence to stationary points of the energy (local minima or saddle points). %They propose hopfield layers which can be integrated in different neural network architectures. \andre{maybe 1 brief sentence explaining how our work differs/relates?}
Like that model, UNNs also seek local minima of an energy function, albeit with a different goal. 

\paragraph{Deep models as graphical model inference.}
This line of work defines neural computation via approximate inference in
graphical models.
%Earlier works also propose new neural network architectures derived from graphical model inference. 
\citet{domke2012optimizationbasedlearning} derives backpropagating versions of gradient descent, heavy-ball and LBFGS. They require as input only routines to compute the gradient of the energy with respect to the domain and parameters. 
\citet{domke2012optimizationbasedlearning} studies learning with unrolled gradient-based inference in general energy models.
UNNs, in contrast, allow efficient, learning rate free, block-coordinate optimization by design.
%focuses on the multi-level optimization problem which we tackle with unrolled coordinate gradient, they tackle with 
% \citet{lawson2019energyinspiredmodels} propose a class of energy-inspired models that incorporate learned energy functions while still providing exact samples and tractable log-likelihood lower bounds.
An exciting line of work derives unrolled architectures
from inference in specific generative models
\citep{hershey2014deepunfolding,li2014meanfieldnetworks,lawson2019energyinspiredmodels}---a powerful construction at the cost of more
challenging optimization. 
The former is closest to our strategy, but by starting from probabilistic models the resulting updates are farther from
contemporary deep learning (\eg, convolutions, attention). In contrast, UNNs can reuse successful implementations, modular pretrained models, as well as structured factors, as we demonstrate in our parsing experiments.
We believe that our UNN construction
%multilinear-regularized factor graph perspective 
can shed new light over probabilistic inference models as well, uncovering deeper connections between the paradigms.

%is close to our work, but motivated by probabilistic modeling it requires more challenging optimization, whereas our construction allows for closed form coordinate gradient updates.
%share our factor graph motivations but focus on pairwise MRFs with binary variables.
%has a similar motivation of designing energy functions for efficient inference, but they are motivated by generative models while we are motivated by parallels to expressive deterministic deep models.
%\citet{li2014meanfieldnetworks} share our factor graph motivations but focus on pairwise MRFs with binary variables.

%\citet{lawson2019energyinspiredmodels} has a similar motivation of designing energy functions for efficient inference, but they are motivated by generative models while we are motivated by parallels to expressive deterministic deep models.
% \citet{hershey2014deepunfolding} combine model-based approach and an associated inference algorithm, and unfold the inference iterations as layers in a deep network. They untie the model parameters across layers, in order to create a more powerful network. This work is closest to ours but is motivated by probabilstic modeling. It requires more challenging optimization, whereas our construction allows for closed form coordinate descent updates.
% \citet{li2014meanfieldnetworks} propose mean field networks, based on a feed-forward network view of the mean field algorithm with fixed number of iterations. 
% \citet{li2014meanfieldnetworks} propose a feed-forward network view of the mean field algorithm with fixed number of iterations. 
%\citet{li2014meanfieldnetworks} share our factor graph motivations but focus on pairwise MRFs with binary variables.
%Our deterministic construction can more easily extend to coarse structured variables or continuous ones.
% \citet{hershey2014deepunfolding} combine a model-based approach and an associated inference algorithm, by unfolding the inference iterations as layers in a deep network. It is motivated by probabilistic modeling and require more challenging optimization, whereas our construction allows for closed form coordinate descent updates.
%\citet{hershey2014deepunfolding} is close to our work, but motivated by probabilistic modeling it requires more challenging optimization, whereas our construction allows for closed form coordinate gradient updates.


% \citep{domke2012optimizationbasedlearning, li2014meanfieldnetworks, hershey2014deepunfolding, lawson2019energyinspiredmodels}.


% \vlad{like Andre pointed out last week, it "resembles" when you squint, but it is not at all the same, so perhaps we say something like "resembles -- but is different from --".}




==> [ICML 2022] Undirected Neural Networks/unn.tex <==
\section{Undirected Neural Networks}\label{section:unn}

% \andre{you're listing particular cases of UNNs but you haven't defined them yet. here's a sketch of a definition: Let $\mathcal{G} = (V, F)$ be a factor graph, i.e., a bipartite graph consisting of a set of variable nodes $V$ and a set of factor nodes $F$, where each factor node $f \in F \subseteq 2^V$ is linked to a subset of variable nodes. Each variable node $v \in V$ is a associated with a representation vector $x_v$. We define variable (unary) and factor (higher-order) local energy functions $E_v(x_v)$ and $E_f(x_f)$, where $x_f$ is short notation for $(x_v)_{v \in f}$. An assignment of variables defines a total energy function $E(x) = \sum_v E_v(x_v) + \sum_f E_f(x_f)$. Then we need to say that some of these variables are input variables (observed), others are output variables, and the rest are hidden variables.}

% \andre{we need to decide if we're using boldface notation for vectors or not. I'm OK with not using it, but if so we need to remove the bolds from this section}

Let $\mathcal{G} = (V, F)$ be a factor graph, \textit{i.e.}, a bipartite graph consisting of a set of variable nodes $V$ and a set of factor nodes $F$, where each factor node $f \in F \subseteq 2^V$ is linked to a subset of variable nodes.
%
%
%Using our new notation
Each variable node $\var{X} \in V$ is associated with a representation vector $x \in \mathbb{R}^{d_\var{X}}$. 
We define unary energies for each variable
$E_\var{X}(x)$,
as well as higher-order energies 
$E_f(x_f)$, where $x_f$ denotes the values of all variables linked to factor
$f$. Then, an assignment defines a total energy function 
\begin{equation}\label{eq:energy}
E(x_1, \ldots, x_n) \coloneqq \sum_i
E_{\var{X}_i}(x_i) + \sum_f E_f(x_f).
\end{equation}
For simple factor graphs where there is no ambiguity, we may refer to factors
directly by the variables they link to. For instance, a simple fully-connected
factor graph with only two variables $\var{X}$ and $\var{Y}$ is fully specified
by 
%\begin{equation}
$E(x, y) = E_\var{X}(x) + E_\var{Y}(y) + E_\var{XY}(x,y)\,.$
%\end{equation}

The energy function in \cref{eq:energy} induces preferences for certain
configurations. For instance, a globally best configuration can be found by
solving
$\argmin_{x,y} E(x,y)$,
while a best assignment for $\var{Y}$ given a fixed value of $\var{X}$
can be found by solving $\argmin_{y} E(x,y)$.%
\footnote{In this work, we only consider deterministic inference in factor
graphs. Probabilistic models are a promising extension.} %
We may think of, or suggest using notation, that $\var{X}$ is an \emph{input}
and $\var{Y}$ is an \emph{output}. However, intrinsically, factor graphs are not
attached to a static notion of input and output, and instead can be used to
infer any subset of variables given any other subset.

In our proposed framework of UNNs, 
%we define neural networks as factor graphs, where each variable
we define the computation performed by a neural network  
using a factor graph, where each variable is a representation vector (\eg, analogous to the output of a layer in a standard network.)
%\vlad{it is not clear what is a variable in the network. Perhaps we should say <each hidden activation layer is a variable in a factor graph>? this is a crucial paragraph} \andre{or ``each representation vector''}
%in the network is presented as a node in the factor graph. We connect the related variables with factors and define energies for each variable and factor. 
We design the factor energy functions depending on the type of each variable and the desired relationships between them. 
%Our goal is to decrease the model energy with multiple iterations of coordinate descent, i.e. optimizing the energy for one variable at a time. One iteration consists of updating all variables once. We can perform one or multiple iterations, which we mark with $k$. 
%\vlad{I wouldn't say <our goal is to decrease energy with CD>. The way I see it more is: an UNN specifies the relatioships between network layers. To compute the actual activations, we must find configurations that minimize energy. We next show how a specific design of the factor energy functions enables an efficient coordinate descent algorithm and recovers standard feed forward networks when the optimization is truncated at one iteration.}
%\tsvm{Vlad noticed we were not introducing the UNNs clearly. Is this description OK or does it need rework?}.
Inference is performed by minimizing the joint energy with respect to all unobserved variables (\ie, hidden and output values). 
For instance, to construct a supervised UNN, we may designate a particular variable as ``input'' $\var{X}$ and another as ``output'' $\var{Y}$, alongside several hidden variables $\var{H}_i$,  compute
\begin{equation}\label{eq:inference}
\hat{y} = \arg\min_{y} \min_{h_1, \ldots, h_n} E(x, h_1, \ldots, h_n, y)\,,
\end{equation}
and train by minimizing some loss $\ell(\hat{y}, y)$.
However, UNNs are not restricted to the supervised setting or to a single input and output, as we shall explore.

While this framework is very flexible, \cref{eq:inference} is a 
non-trivial optimization problem. Therefore, we focus on
a class of energy functions that renders inference easier: 
\begin{equation}\label{eq:multilinear}
\begin{aligned}
E_{\var{X}_i}(x_i) &= -\DP{b_{\var{X}_i}}{x_i} + \Reg_{\var{X}_i}(x_i)\,,\\
E_{f}(x_f) &= -\bigDP{W_f}{\bigotimes_{\var{X}_j \in f} x_j }\,, \\
\end{aligned}
\end{equation}
where each $\Reg_{\var{X}_i}$ is a strictly convex regularizer, 
$\otimes$ denotes the outer product, and $W_f$ is a parameter tensor
of matching dimension.
For pairwise factors $f = \{\var{X}, \var{Y}\}$, the factor energy 
is bilinear and can be written simply as $E_{\var{XY}}(x, y) = -x^\top W y$.
In factor graphs of the form given in \cref{eq:multilinear}, the energy is convex in each variable separately, and block-wise minimization has a closed-form expression involving the Fenchel conjugate of the regularizers. This suggests a block coordinate descent optimization strategy: given an order $\pi$, iteratively set:
\begin{equation}\label{eq:coordinate_descent}
x_{\pi_j} \leftarrow \argmin_{x_{\pi_j}}~E(x_1, \ldots, x_n)\,.
\end{equation}
This block coordinate descent algorithm is guaranteed to decrease energy at every iteration and, for energies as in \cref{eq:multilinear}, to converge to a Nash equilibrium \citep[Thm.~2.3]{xu2013block}; in addition, it is conveniently learning-rate free. 
%At each step one variable is updated with coordinate descent and there can be multiple steps of energy optimization. Since coordinate descent is used, it is guaranteed that the total model energy will decrease with each step (\citet{bertsekasnonlinear}, Proposition 2.7.1).
For training, to tackle the bi-level optimization problem, we unroll the coordinate descent iterations, 
%With energies of the form in \cref{eq:multilinear}, this yields a standard computation graph (\cref{fig:unroll_undirected_mlp}), over which 
and minimize some loss with standard deep learning optimizers, like stochastic gradient or Adam \citep{kingma2014adam}.

%Some of these variables are input variables (observed), others are output variables (to be predicted), and the rest are hidden variables. In the examples below, we will denote the
%input variable with $\var{X}$, the output variable with $\var{Y}$ and the hidden variables with other letters (and indices, where applicable).

% \vlad{This definition so far is a definition of *factor graphs*, not of undirected neural networks. What is an undirected neural network?}

%On inference, the goal is to optimize the model energy.
% \vlad{what model?}

The following result, proved in \cref{sec:proof_lemma_unrolling}, shows that the coordinate descent algorithm (\cref{eq:coordinate_descent}) for UNNs with multilinear factor energies (\cref{eq:multilinear}), corresponds to standard forward propagation on an unrolled neural network.  
\begin{lemma}[Unrolling Lemma]\label{lemma:unrolling}
Let $\mathcal{G} = (V,F)$ be a pairwise factor graph, with multilinear higher-order energies and strictly convex unary energies, as in \cref{eq:multilinear}. 
Then, the coordinate descent updates \eqref{eq:coordinate_descent} result in a chain of affine transformations (\textit{i.e.}, pre-activations) followed by non-linear activations, applied in the order $\pi$, yielding a traditional computation graph.
\end{lemma}

%\andre{I added a proof to this lemma (actually a more general version of it. The proof is long and should be moved to the appendix, but for now I'm leaving it here since we might want to use some of the notation here to explain better what UNNs are and how (block) coordinate descent works.}

%\vlad{my favorite thing here is how you introduce the analogy with <preactivations> to build familiarity, nice!}

We show next an undirected construction inspired by (directed) multi-layer perceptrons.

% \andre{We need to describe here how inference works in our model: that the goal is to minimize the energy.}

%\paragraph{Network without intermediate layers}

\paragraph{Single pairwise factor}

%\vlad{I think Andre said on Friday that this section title is unclear}

% \andre{Maybe we could move this example before the standard NN one? It's the simplest thing we can get, a graph with two variables and one factor. We could bring it right after the UNN definition and say that it corresponds to a Boltzmann-like machine with continuous variables (another particular case of our framework) -- or maybe there is a better name? the main difference is that we don't use the BM    to define a distribution $p(x,h) \propto \exp(-E(x,h))$ but we only care about modes, e.g., $h^\star(x) = \arg\max_h p(h|x) = \arg\min_h E(x,h)$}

The simplest possible UNN has a pairwise factor connecting two variables $\var{X,H}$. 
We may interpret $\var{X}$ as an input, and
$\var{H}$ either as an output (in supervised learning) or a hidden representation in unsupervised learning (\cref{fig:factors_all_models}(a)). 
%
% \begin{figure}{t}
%     \centering
%     \includegraphics[width=5cm]{img/factor_x_h.png}
%     \caption{Factor graph representing a network with visible and hidden units. }
%     \label{fig:factor_x_h}
% \end{figure} 
% \andre{The key thing here is that we define a factor energy which is bilinear.} 
Bilinear-convex energies as in \cref{eq:multilinear} yield:
\begin{equation}\label{eq:energy_rbm}
\begin{aligned}
E_{\var{XH}}(x,h) &= -\DP{h}{Wx}\,,\\
E_\var{X}(x) &= -\DP{x}{b_\var{X}} + \Reg_\var{X}(x)\,,\\
E_\var{H}(h) &= -\DP{h}{b_\var{H}} + \Reg_\var{H}(h)\,.\\
\end{aligned}
\end{equation}
This resembles a Boltzmann machine with continuous variables \citep{smolensky1986information,hinton2007boltzmann,welling2004exponential}; %; in particular, with Euclidean norm regularizers, a Gaussian RBM\vlad{defined?}, demonstrating how such models fit in our framework.
however, in contrast to  Boltzmann machines, we do not
model joint probability distributions,
but instead use factor graphs as representations 
of deterministic computation, more akin to computation graphs.
%% but instead \emph{computation}
%% (another particular case of our framework). The main difference is that we do not use this representation to define a distribution $p(x,h) \propto \exp(-E(x,h))$ (as done with Boltzmann machines), but we only care about modes, \textit{e.g.}, $h_\star(x) = \arg\max_h p(h|x) = \arg\min_h E(x,h)$.

Given ${x}$,
the updated $h$ minimizing the energy is:
\begin{equation}
\begin{aligned}
    {h}_\star &= \argmin_{h \in \reals^{M}} -(W\currit{x}+b_\var{H})^{\top}h + \Reg_\var{H}(h) \\
    &= (\nabla \Reg_\var{H}^{*})(Wx+b_\var{H}),
\end{aligned}
\end{equation}
where $\nabla \Reg_\var{H}^{*}$ is the gradient of the conjugate function of $\Reg_\var{H}$. 
% \andre{We need to explain here what $B^*$ and $\nabla B^*$ are. We should probably assume that $B$ is convex. Then we can point to the table for the examples.} \tsvm{Is the explanation below meaningful and understandable?} 
% \andre{Perhaps we can also describe the $x^\star(h)$ when $h$ is given. We could point out that there two iterations, when done consecutively, describe the computation of an auto-encoder.} 
% \vlad{I think there's a notation problem here: the star in $h^*$ means ``optimal'', right? but the star in $B^*$ means conjugate? If yes, you're supposed to differentiate these. You can use $h^\star$ for optimum instead, for instance. (A paper I'm reading now uses $h_*$ which i kind of like too, but it's more surprising.} 
% The total energy of the network is $E_{X,H}(h, x) + E_{X}(x) + E_{H}(h)$. 
% Then we have $h^\star = argmin_{h} -(h^{\top} W x) + c - h^{\top} b + B(h)$  which we can rewrite as $min_{h} -h^{\top} (Wx + b) + B(h)$. 
%To see why, note that, since $x$ is given, then the optimization is over $h$ only, then $E_{\var{X}}(x)$ is constant.
% and we can set it to $c$.
%If we set $z = Wx+b$, then we want to minimize $\Reg_\var{H}^{*}(z) = \min_h \Reg_\var{H}(h) - h^{\top} z$.
%This is the optimization problem that we need to solve in order to find the best $h$ for a given z (i.e. for a given x).
%$\nabla \Reg_\var{H}^{*}$ is the gradient of the conjugate function of $\Reg_\var{H}$. 
Analogously, the update for $\var{X}$ given $\var{H}$ is:
\begin{equation}
    \begin{aligned}
    \nextit{x}
%&= \argmin_{x \in R^{N}} -(\currit{h}^{\top}W + a)\currit{x} + \Reg_x(\currit{x}) \\
    &= (\nabla \Reg_\var{X}^{*})(W^\top\currit{h}+ b_\var{X})\,.
\end{aligned}
\end{equation}
Other than the connection to Boltzmann machines,
one round of updates of $\var{H}$ and $\var{X}$ in this order
also describe the computation of an auto-encoder with shared encoder/decoder weights. %
%\footnote{In particular, with $b_\var{X} = b_\var{H} = 0$ and $\psi_\var{X} = \psi_\var{X} = \frac{1}{2}\|\cdot\|^2$, coordinate descent converges in a single iteration; minimizing a squared error loss on a given dataset recovers  principal component analysis.}
% \vlad{as well as a round of mean-field inference in a RBM?}. 

\cref{table:unn_functions} shows examples of regularizers $\Reg$ and their corresponding $\nabla \Reg^{*}$,
In practice, we never evaluate $\Reg$ or $\Reg^*$, but only $\nabla \Reg^*$, 
which we choose among commonly-used neural network activation functions like $\tanh$, $\relu$, and $\softmax$.

\begin{table}[t]
    \renewcommand\arraystretch{1.5}%
    \centering%
    \caption{\label{table:unn_functions} Examples of regularizers $\Reg(h)$
corresponding to some common activation functions,
where $\phi(t) = t \log t.$}
    \vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{ll}
    \toprule
    $\Reg(h)$ & $(\nabla \Reg^{*})(t)$  \\
    \midrule
    %$\frac{1}{2}||h||^2 + \iota_{\Delta}(h)$ & $\sparsemax(t)$ \\
    % \midrule
    $\frac{1}{2} \| h \|^2$ & $t$ \\
    % \midrule
    $\frac{1}{2}\| h \|^2 + \iota_{\reals_{+}}(h)$ & $\relu(t)$ \\
    % \midrule
    $\sum_{j}\!\big(\phi(h_j) + \phi(1-h_j)\big) + \iota_{[0,1]^d}(h)$ &
$\operatorname{sigmoid}(t)$\\
    % \midrule
    $\sum_{j}\!\left(\phi\left(\frac{1+h_j}{2}\right)
    +\phi\left(\frac{1-h_j}{2}\right)\right)
+ \iota_{[-1,1]^d}(h)$ & $\tanh(t)$ \\
    % \midrule
    $-\entropy(h) + \iota_{\Delta}(h)$ & $\softmax(t)$ \\
    \bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{img/unroll_undirected_mlp.pdf}
    \caption{Unrolling the computation graph for undirected MLP with a single hidden layer. Top: MLP with one hidden layer. Bottom: Unrolled graph for UNN with $k=3$ iterations.}
    \label{fig:unroll_undirected_mlp}
\end{figure}


\paragraph{Undirected multi-layer perceptron (MLP)}
\cref{fig:factors_all_models}(b) shows the factor graph for an undirected MLP
analogous to a feed-forward one with input $\var{X}$, output $\var{Y}$,
and a single hidden layer $\var{H}$. 
As in \cref{eq:multilinear}, we have bilinear pairwise factors
\begin{equation}
    E_\var{XH}(x,h) = -\DP{h}{Wx}\,, \quad 
    E_\var{HY}(h,y) = -\DP{y}{Vh}\,,
\end{equation}
and linear-plus-convex unaries
$E_\var{Z}(x) = -\DP{x}{b_\var{Z}} + \Reg_\var{Z}(x)$
for $\var{Z}\in\{\var{X},\var{H},\var{Y}\}$.
If $x$ is observed (fixed), coordinate-wise
inference updates take the form:
\begin{equation}
\begin{aligned}
    \nextit{h} 
    &= 
     (\nabla \Reg_\var{H}^{*})(Wx+V^{\top}\currit{y}+b_\var{H})\,, \\
    \nextit{y} 
    &= 
     (\nabla \Reg_\var{Y}^{*})(V{h}+b_\var{Y})\,.
\end{aligned}
\end{equation}
Note that $E_\var{X}$ does not change anything if $\var{X}$ is always observed.
The entire algorithm
can be unrolled into a directed computation graph, leading to a deep neural
network with shared parameters (\cref{fig:unroll_undirected_mlp}). 

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{img/factors_all_models.pdf}
    \caption{Factor graphs for:
    (a) network without intermediate layers,
    (b-c) undirected MLPs with one or two layers,
    (d) undirected biaffine dependency parser,
    (e) undirected self-attention.
Energy labels ommitted for brevity with the exception of (d).
    }
    \label{fig:factors_all_models}
\end{figure*}


The regularizers $\Reg_\var{H}$ and $\Reg_\var{Y}$ may be selected based on what
we want $\nabla\Reg^*$ to look like, and the constraints or domains of the
variables. For instance, if $\var{Y}$ is a multiclass classification output,
we may pick $\Reg_\var{Y}$ such that
$\nabla\Reg_\var{Y}^*$ be the softmax function,
and $\Reg_\var{H}$ to induce a relu nonlinearity.  
Initializing $\initit{y}=0$ and performing a single iteration of updating $\var{H}$ followed by $\var{Y}$ results in a standard MLP with a single hidden layer (see also \cref{fig:unroll_undirected_mlp}).
However, the UNN point of view lets us decrease energy further by performing multiple iterations,
as well as use the same model to infer any variables given any other ones, \textit{e.g.}, to predict $x$ from $y$ instead of $y$ from $x$.
We demonstrate this power in
\cref{section:experiments_mnist,section:experiments_attention,section:experiments_parsing}.




The above constructions provide a flexible framework for defining UNNs. However, UNNs are more general and cover more popular deep learning architectures. The following constructions illustrate some such connections.

\paragraph{Feed-forward neural networks}
% \vlad{Here, make it clear that this is *not* our construction, but an example.}

Any directed computation graph associated with a neural network is a particular case of an UNN. We illustrate this for a simple feed-forward network, which chains the functions $h = f(x)$ and $y = g(h)$, where $x \in \reals^m$, $h \in \reals^d$, $y \in \reals^n$ are input, hidden, and output variables, and $f: \reals^m \rightarrow \reals^d$ and $g: \reals^d \rightarrow \reals^n$ are the functions associated to each layer (\textit{e.g.}, an affine transformation followed by a non-linearity). This factor graph is illustrated in \cref{fig:factors_all_models}(b).
To see this, let $V = \{\var{X}, \var{H}, \var{Y}\}$ and $F = \{\var{XH},\var{HY}\}$ and define the energies as follows.
Let $d: \reals^d \times \reals^d \to \reals_+$ be any distance function satisfying $d(a,b) \ge 0$, with equality iff $a = b$; for example $d(a,b) = \|a-b\|$.
Let all the unary energies be zero and define the factor energies
$E_{\var{XH}}(x, h) = d(h,f(x))$ and $E_{\var{HY}}(h, y) = d(y,g(h))$. Then
the total energy satisfies $E(x, h, y) \ge 0$, with equality iff the
equations $h = f(x)$ and $y = g(h)$ are satisfied -- therefore, the energy is
minimized (and becomes zero) when $y=g(f(x))$, matching the corresponding directed computation graph.
This can be generalized for an arbitrary deterministic neural network. 
This way, we can form UNNs that are partly directed, partly undirected, as the whole is still an UNN. We do this in our experiments in \cref{section:experiments_parsing}, where we fine-tune a pretrained BERT model appended to a UNN for parsing.

% It is straightforward \vlad{avoid this phrase at all costs!!!} to generalize this for an arbitrary deterministic neural network.

%We define a distance function $d : R^{N} R^{M} \rightarrow R_{+}$ such that $d(a, b) = 0 \Leftrightarrow a = b$.
%We can create a factor with energy: $E_{X,H}(x,h) = d(h,f(x))$.
%The energy is minimized when the computation graph is executed, resulting in an energy of zero.
%Directed neural networks are a particular case of this construction.


\paragraph{Implicit layers}
% \vlad{Make the connection that we can represent networks with implicit layers by picking $E_{XH}$ accoringly.}
UNNs include networks with implicit layers
\citep{duvenaud2020deep}, a paradigm which, in contrast with feed-forward
layers, does not specify how to compute the output from the input, but rather
specifies conditions that the output layer should specify, often related to
minimizing some function, \eg, computing a layer $h_{i+1}$ given a previous
layer $h_{i}$ involves solving a possibly difficult problem $\argmin_{h} f(h_i, h)$.
Such a function $f$ can be directly interpreted as an energy in our model, \ie,
$E_{\var{H}_i\var{H}_{i+1}} = f$.
% \vlad{compare this paragraph with the notation from Duvenaud, make more similar}\tsvm{changed the $f$ only}
% \vlad{I think what Andre means is that if in our framework we pick $E_{XH}$ to be some more complicated function of $x$ and $h$ (not simply a bilinear + pointwise penalty one) then computing $h^\star$ given $x$ is an "implicit layer" that requires optimization. So I think our formalism does "subsume" implicit layers, although none of our concrete experiments use this. We should explain this connection somewhere in text.}




==> _experiments_multitask.tex <==
\section{Multitask Learning}

\andre{I promoted this to section}

\andre{so far the results for this task are not  compelling. consider dropping this.}

We also explore UNN for multiple tasks. Figure \ref{fig:factor_graph_multitask} shows the factor graph for a simple multitask setup. 
 
This graph resembles the directed neural network for multitasking. The difference is that for multiple iterations, UNNs can be more powerful for identifying relations between the multiple task labels. When we have more iteration updates,  

 
\begin{figure*}
    \centering
    \includegraphics[width=12cm]{img/factor_graph_multitask.png}
    \caption{Factor graph for a UNN for multiple tasks.}
    \label{fig:factor_graph_multitask}
\end{figure*}



Here we have the following energies:

\begin{equation}
    E_{X,H}(x,h) = -h^{T}Wx
\end{equation}

\begin{equation}
    E_{H,Y_1}(h,y_1) = -y_1^{T}Vh
\end{equation}

\begin{equation}
    E_{H,Y_2}(h,y_2) = -y_2^{T}Uh
\end{equation}

\begin{equation}
    E_{X}(x) = -a^{T}x + A(x)
\end{equation}

\begin{equation}
    E_{H}(h) = -b^{T}h + B(h)
\end{equation}

\begin{equation}
    E_{Y_1}(y_1) = -c^{T}y_1 + C(y_1)
\end{equation}

\begin{equation}
    E_{Y_2}(y_2) = -d^{T}y_2 + D(y_2)
\end{equation}

We minimize the model with respect to $h$, $y_1$, $y_2$ iteratively. 

\begin{equation}
\begin{split}
    h^\star(x,y) = \\
    \argmin_{h}(E(h) + E(x,h) + E(h,y_1) + E(h,y_2)) \\
    = \argmin_h(-b^{T}h + B(h) \\
    - h^{T}Wx - y_1^{T}Vh - y_2^{T}Uh) \\
    = (\nabla B^{*})(Wx + V^{T}y_1 + U^{T}y_2 + b)
\end{split}
\end{equation}

\begin{equation}
\begin{split}
    y_1^{*}(x,h) = \argmin_{y_1}E(h,y_1) \\
    = (\nabla C^{*})(Vh+b_1)
\end{split}
\end{equation}

\begin{equation}
\begin{split}
    y_2^{*}(x,h) = \argmin_{y_2}E(h,y_2) \\
    = (\nabla D^{*})(Uh+b_2)
\end{split}
\end{equation}




We experiment how the multiple updates of energy optimization can benefit when the model is trained for multiple tasks. For this experiment, we use the architecture described in Section~\ref{section:multitask_unn}. 
We use dataset with movie reviews from IMDB \citep{maas-EtAl:2011:ACL-HLT2011}. On of the tasks is classification of the review sentiment. For the second task, inspired by \citet{zhang2021disentangling}, we add the movie genre as a second related task. Ass described in \citet{zhang2021disentangling}, we use movies with genre Horror and Drama, because as this work shows, the review sentiment is correlated with those two genres. Because the genre is not present in the original dataset, we use the movie genres from the IMDB website. \footnote{https://www.imdb.com/interfaces/, file: \textbf{title.basics.tsv.gz}} The reviews in \citet{maas-EtAl:2011:ACL-HLT2011} contain the movie ID from IMDB and by this ID we match the movie genre. We only use the reviews with genre Drama or Horror (excluding the few cases where both labels are present). The training split from the original dataset is kept, and the test split from the original dataset is split randomly into validation and test set. The number of instances is shown on Table~\ref{table:multitask_data}.

\begin{table}[]
    \centering
    \caption{Number of instances in the training and development split for multitask data on IMDB movie reviews sentiment and genre classification.}
    \begin{tabular}{c|c|c}
        \toprule
         \multicolumn{3}{c}{Train}  \\
         \midrule
         & Drama & Horror \\ 
         \midrule
         Positive & 6111 & 897 \\ 
         Negative & 4412 & 2650 \\
         \midrule
         \multicolumn{3}{c}{Test}  \\
         \midrule
         & Drama & Horror \\ 
         \midrule
         Positive & 6100 & 1055 \\ 
         Negative & 4488 & 2599 \\ 
    \end{tabular}
    \label{table:multitask_data}
\end{table}

The input of the model is the review text and the two tasks we predict are the review sentiment and the genre of the movie this review is written for. 
The movie review is passed through a BERT (we use \emph{BERT-Tiny} \tsvm{cite}) and is used as the input $x$, and the architecture is as described in Section~\ref{section:multitask_unn}.
We run a baseline for each task, where the model is run only for the specific task and the weights are updated for that task only. The idea is to validate our assumption that adding a second task would improve the result of the first task (sentiment classification). When multiple energy updates are executed, the tasks inform one another and we expect to see improvement if the tasks are correlated.

We fine-tune the learning rate and use a value of 0.0001. We also fine-tuned the weight between the two tasks and end up with a weight 0.6 for the sentiment and 0.4 for the genre task.

Table~\ref{table_multitask_results} shows the results from the experiments. We show the average of 5 runs for the UNN. The results show that training both tasks together and having more energy update iterations improves the prediction of the first task (sentiment classification).

\begin{table*}[]
    \centering
    \caption{Results from multitask learning - sentiment and genre classification of IMDB movie reviews. \andre{are these results up-to-date?}}
    \begin{tabular}{c|c|c}
         & Accuracy Sentiment & Accuracy Genre \\
         Baseline Sentiment & 77.63 & \-- \\
         Baseline Genre & \-- & 89.77 \\
         Baseline Both (UNN with k=1) & 79.43 & 88.51 \\
         Both, k=2 & 75.72 & 88.41 \\
         Both, k=3 & \textbf{80.56} & 88.51 \\
         Both, k=4 & 78.75 & 87.48 \\
         Both, k=5 & 79.66 & 88.46 \\
    \end{tabular}
    \label{table:multitask_results}
\end{table*}

\tsvm{TODO: We also make the assumption that in test time, when the gold label for one of the tasks is given, this leads to improving the prediction of the other task. i.e. in this case, when predicting sentiment, we pass the gold label of the genre and expect the multiple updates to lead to improved prediction of the sentiment.}



==> background.tex <==
% Energy-Based Models capture dependencies by associating a scalar energy (a measure of compatibility) to each configuration of the variables in a model. 
% Inference, i.e., making a prediction or decision, consists in setting the value of observed variables and finding values of the remaining variables that minimize the energy. Learning consists in finding an energy function that associates low energies to correct values of the remaining variables, and higher energies to incorrect values. A loss function, minimized during learning, is used to measure the quality of the available energy functions \citep{lecun2006tutorial}.

% Let us consider a model with two sets of variables, $x$ and $y$. Following the examples of NLI \andre{not defined so far. consider replacing by a different example in case we don't do NLI in the paper}, variable $x$ could be a representation of the premise and hypothesis. Variable $y$ could be a discrete variable that represents the possible category of the object. For example, in the NLI case $y$ could take three possible values: entailment, contradiction, neutral. The model is viewed as an energy function which
% measures how good each configuration of $x$ and $y$ is. The output number (i.e. the energy) can be interpreted as a measure of how much $x$ and $y$ are compatible. 

% Small energy would mean that the variables are highly compatible and vice versa.  The energy function is denoted as $E(x,y)$.

% In the energy-based model, the input $x$ is given (observed), and the model produces the $y$ that is most compatible with the observed $x$ \citep{lecun2006tutorial}. 
% As a result, we would like to find $y^{*}$
% , chosen from a set $Y$, for which
% $E(x,y)$ is the smallest:
% $y^{*} = \argmin_{y} E(x,y)$ \andre{I think we can keep only this paragraph and delete the previous two. Maybe rephrase as ``An energy-based model is a network which takes as inputs $x$ (observed) and $y$ (a candidate output from a set $\mathcal{Y}$) and computes an energy function $E_\theta(x,y)$, which defines the compatibility between $x$ and $y$. The goal is to the predict $y^{*} \in \mathcal{Y}$ that minimizes the energy, $y^{*} = \argmin_{y} E_\theta(x,y)$. This corresponds to the most probable output under a Gibbs distribution, $p_\theta(y \mid x) \propto \exp(-E_\theta(x,y))$, avoiding modeling this distribution explicitly.''}

An energy-based model is a network which takes as inputs $x$ (observed) and $y$ (a candidate output from a set $\mathcal{Y}$) and computes an energy function $E_\theta(x,y)$, which defines the compatibility between $x$ and $y$. The goal is to the predict $y^{*} \in \mathcal{Y}$ that minimizes the energy, $y^{*} = \argmin_{y} E_\theta(x,y)$. This corresponds to the most probable output under a Gibbs distribution, $p_\theta(y \mid x) \propto \exp(-E_\theta(x,y))$, avoiding modeling this distribution explicitly.

\subsection{Hopfield Networks}
% \andre{This subsection can be trimmed a bit and potentially moved to the related work section, unless it makes it easier for us to explain our UNNs. Also this definitions are not distinguishing between Hopfield and Boltzmann networks, right?}
Hopfield networks \citep{hopfield1982neural} consist of binary units with symmetric, bidirectional connection weights between them, i.e. each unit is connected to all other units \citep{stone2019artificial}. The total input to a unit depends on the states of all other units.
The energy function is  defined for every possible set of unit states and the total energy is the sum of the energies of all units.

% The energy function is  defined for every possible set of unit states by the formula:

% \begin{equation}
%     E(y) = -\sum_{i=1}^{K}\sum_{j=i+1}^{K}w_{ij}y_{i}y_{j}
% \end{equation}

% where $w$ are the weights, $y$ are the states of the units and $K$ is the number of units.

% The energy contributed by a single unit is:

% \begin{equation}
%     E_{i} = -y_{i}\sum_{j=1}^{K}w_{ij}y_{j}
% \end{equation}

% And the total energy is the sum of the energies of all units:

% \begin{equation}
%     E(y) = \sum_{i=1}^{K}E_{i}
% \end{equation}

% The energy function is derived  from statistical mechanics, where it is called the Hamiltonian; in  optimisation theory it is called a Lyapunov function \citep{stone2019artificial}.

% The continuous Hopfield networks \citep{hopfield1984neurons} 

% Recent work \citep{ramsauer2020hopfield} shows that the attention mechanism of the widely used Transformer model \citep{vaswani2017attention} is equal to the update rule of a Hopfield network with continuous states \citep{hopfield1984neurons}. 


\subsection{Boltzmann Machines}

% \andre{this section can also be trimmed, we don't need to have special subsections for RBMs and DBMs and write all the equations, we only need to mention them briefly.} 
A Boltzmann Machine \citep{ackley1985learning} is a network of symmetrically connected, neuronlike units that make stochastic decisions about whether to be on or off. Boltzmann machines have a simple learning algorithm that allows them to discover
interesting features in datasets composed of binary vectors. The learning algorithm is intractable in networks with many layers of features. \citep{hinton2007boltzmann}
% detectors, but it can be made much faster by learning one layer of  feature detectors at a time. \citep{hinton2007boltzmann}

% Boltzmann machines are pairwise fully connected neural
% networks with N visible units $x \in \{0, 1\}^{N}$ and M hidden units $x \in \{0, 1\}^{M}$.
% They define the following energy function:

% \begin{equation}
% E(x, h) = -x^{T}Rx - h^{T}Wx - h^{T}Sh - a^{T}x - b^{T}h
% \end{equation}

% The probability of a configuration is defined as:

% \begin{equation}
% P(x, h) = \frac{\exp(-E(x, h))}{Z}
% \end{equation}

% \noindent(where Z is the partition function)
% and maximizing the probability corresponds to minimizing the energy. We can represent a Boltzmann machine with the factor graph diagram in Figure 1, defining a bilinear factor energy

% \begin{equation}
%     E_{x, h}(x, h) = - h^{T}Wx
% \end{equation}

% \noindent and unary energies

% \begin{equation}
%     E_{x}(x) = - x^{T}Rx- a^{T}x + \iota_{\{0,1\}^{N}}(x)
% \end{equation}

% \noindent and 

% \begin{equation}
%     E_{h}(h) = - h^{T}Wx - b^{T}h + \iota_{\{0,1\}^{M}}(h)
% \end{equation}

% \noindent $\iota_{\{0,1\}^{N}}(x)$ means that we set constraints for $x$ to be a binary vector with $N$ units.
% \vlad{define this more clearly in the notations section}


% \subsection{Restricted Boltzmann Machines} 
% Restricted Boltzmann machines are special cases of Boltzmann machines where the connections between visible and hidden units form a bipartite graph. In this case, we have:

% \begin{equation}
%     E_{X, H}(x, h) = - h^{T}Wx
% \end{equation}

% \begin{equation}
%     E_{X}(x) = - a^{T}x + \iota_{\{0,1\}^{N}}(x)
% \end{equation}

% \begin{equation}
%     E_{H}(h) = - b^{T}h + \iota_{\{0,1\}^{M}}(h)
% \end{equation}


% \subsection{Deep Boltzmann Machines} 
% Deep Boltzmann machines are similar to restricted Boltzmann machines, but
% with more layers. Here we have:

% \begin{equation}
%     E_{X, H_{1}}(x, h_{1}) = - h_{1}^{T}W_{1}x
% \end{equation}

% \begin{equation}
%     E_{H_{k-1}, H_{k}}(h_{k-1}, h_{k}) = - h_{k}^{T}W_{k}x
% \end{equation}

% \begin{equation}
%     E_{X}(x) = - a^{T}x + \iota_{\{0,1\}^{N}}(x)
% \end{equation}

% \begin{equation}
%     E_{H_{k}}(h_{k}) = - b_{k}^{T}h_{k} + \iota_{\{0,1\}^{M_{h}}}(h_{k})
% \end{equation}



The Boltzmann Machines are pairwise fully connected neural networks with $N$ visible units $x$ and $M$ hidden units $h$. The probability of a configuration is defined as: 

\begin{equation}
    P(x,h) = \frac{exp(-E(x,h))}{Z}
\end{equation}

Maximizing the probability corresponds to minimizing the energy.

\begin{equation}
    E(x,h) = - x^{T}Rx - h^{T}Wx - h^{T}Sh - a^{T}x - b^{T}h
\end{equation}

The total energy is given by:

\begin{equation}
    E(x,h) = E_{X}(x) + E_{H}(h) + E_{X,H}(x,h)
\end{equation}

where

\begin{equation}
    E_{X,H}(x,h) = - h^{T}Wx
\end{equation}

\begin{equation}
    E_{X}(x) = - a^{T}x + \iota_{\{0,1\}^{N}}(x)
\end{equation}

\begin{equation}
    E_{H}(h) = - b^{T}h + \iota_{\{0,1\}^{M}}(h)
\end{equation}

where $\iota_{\{0,1\}^{N}}(x)$ means constraint on $x$, i.e. $x$ needs to be $N$ zeros or ones.
% \vlad{define this more clearly in the notations section}


\textbf{Restricted Boltzmann Machines (RBMs)} are special cases of Boltzmann machines where the connections between visible and hidden units form a bipartite graph. \noindent The separation of visible and hidden units in the RBMs allows for more efficient training algorithms than for the general Boltzmann machines \citep{smolensky1986information,hinton2007boltzmann}. 
\textbf{Deep Boltzmann Machines (DBMs)} are similar to restricted Boltzmann machines, but with more layers.
